Prophet Inequalities via the Expected Competitive Ratio

We consider prophet inequalities under downward-closed constraints. In this problem, a decision-maker makes immediate and irrevocable choices on arriving elements, subject to constraints. Traditionally, performance is compared to the expected offline optimum, called the \textit{Ratio of Expectations} (RoE). However, RoE has limitations as it only guarantees the average performance compared to the optimum, and might perform poorly against the realized ex-post optimal value. We study an alternative performance measure, the \textit{Expected Ratio} (EoR), namely the expectation of the ratio between algorithm's and prophet's value. EoR offers robust guarantees, e.g., a constant EoR implies achieving a constant fraction of the offline optimum with constant probability. For the special case of single-choice problems the EoR coincides with the well-studied notion of probability of selecting the maximum. However, the EoR naturally generalizes the probability of selecting the maximum for combinatorial constraints, which are the main focus of this paper. Specifically, we establish two reductions: for every constraint, RoE and the EoR are at most a constant factor apart. Additionally, we show that the EoR is a stronger benchmark than the RoE in that, for every instance (constraint and distribution), the RoE is at least a constant fraction of the EoR, but not vice versa. Both these reductions imply a wealth of EoR results in multiple settings where RoE results are known.

==> sections/background.tex <==
\section{Background}\label{background}
\subsection{Secretaries, Prophets and Prophet Secretaries}

\noindent \emph{Full-knowledge of Input Distributions.} We formally introduce the models encompassing random and adversarial arrivals, assuming we possess full knowledge of input distributions whenever needed. In all models, variables are assumed to be non-negative and $X_\tau$ represents the value the considered stopping rule $\textbf{r}$ picks.

\begin{model}[Secretary]\label{secretary}
The secretary model is described as follows:
\begin{itemize}
    \item \textbf{Adversary}: Chooses values $X_1, \dots, X_n$.
    \item \textbf{Environment}: Shuffles values $X_1, \dots, X_n$ uniformly at random, i.e. creates a permutation of the form $(X_1, \dots, X_n) \mapsto \pi(X_1, \dots, X_n) = \left(X_{\pi_1}, \dots, X_{\pi_n}\right)$.
    \item \textbf{Objective}: Maximize the probability of selecting the maximum $\Pr\left[X_\tau = \max_{i \in [n]}{X_{\pi_i}} \right]$, where $X_\tau$ is the accepted variable.
\end{itemize}
\begin{align}
    \inf_{X_1, \dots, X_n}{\sup_{\textbf{r}}{\Pr\left[X_\tau = \max_{i \in [n]}{X_{\pi_i}} \right]}}
\end{align}
\end{model}

The secretary model focuses on a uniformly random arrival model on values that are adversarially chosen. When values are not completely adversarial, but are drawn from adversarially constructed distributions, another benchmark comparison is against the expected maximum, i.e. what the prophet could have gotten in expectation.

\vspace{0.2cm}

\begin{model}[Prophet]\label{prophet}
The prophet model is described as follows:
\begin{itemize}
    \item \textbf{Adversary}: Chooses distributions $F_1, \dots, F_n$ and order in which variables $X_1 \sim F_1, \dots, X_n \sim F_n$ are sent to the stopping rule.
    \item \textbf{Environment}: Samples values $X_1 \sim F_1, \dots, X_n \sim F_n$.
    \item \textbf{Objective}: Maximize the ratio between the stopping rule's expected stopping value and the expectation of the maximum $\E\left[X_\tau\right]/\E\left[\max_{i \in [n]}{X_i}\right]$, where $X_\tau$ is the accepted variable.
\end{itemize}
\begin{align}
    \inf_{F_1, \dots, F_n}{\sup_{\textbf{r}}{\frac{\E\left[X_\tau\right]}{\E\left[\max_{i \in [n]}{X_i}\right]}}}
\end{align}
\end{model}

When we want to constrain the adversary, we introduce a model where the environment induces both a random order and samples values from distributions, yet adversarially devised.

\vspace{0.2cm}

\begin{model}[Prophet Secretary]\label{prophet_secretary}
The prophet secretary model is described as follows:
\begin{itemize}
    \item \textbf{Adversary}: Chooses distributions $F_1, \dots, F_n$.
    \item \textbf{Environment}: Samples values $X_1 \sim F_1, \dots, X_n \sim F_n$ and shuffles values $X_1, \dots, X_n$ uniformly at random, i.e. creates a permutation of the form $(X_1, \dots, X_n) \mapsto \pi(X_1, \dots, X_n) = \left(X_{\pi_1}, \dots, X_{\pi_n}\right)$..
    \item \textbf{Objective}: Maximize the ratio between the stopping rule's expected stopping value and the expectation of the maximum $\E\left[X_\tau\right]/\E\left[\max_{i \in [n]}{X_{\pi_i}}\right]$, where $X_\tau$ is the accepted variable.
\end{itemize}
\begin{align}
    \inf_{F_1, \dots, F_n}{\sup_{\textbf{r}}{\frac{\E\left[X_\tau\right]}{\E\left[\max_{i \in [n]}{X_{\pi_i}}\right]}}}
\end{align}
\end{model}

\vspace{0.5cm}

The three models above aim to measure different kinds of performance in single-choice online problems. One might wonder why we did not include a fourth model where both values and their arrival order are \emph{a priori} chosen by the adversary. In this case, the adversary would have complete power over any stopping rule, and in particular every deterministic strategy must fail. Suppose there are only two variables arriving, and the adversary sends $X_1 = 1$. If the stopping rule accepts, then the adversary will send $X_2 = 2$, otherwise $X_2 = 1/2$. Hence, we have no guarantee on the probability of selecting the maximum when the stopping rule we employ is deterministic. Randomization helps but, as shown formally in section \ref{prophet_nosamples}, it cannot push such a probability above $1/n$ for $n$ variables, that is random guessing.\\

\noindent \emph{Sample-access to Input Distributions.}
Up to this point, we have assumed that the stopping rule has full knowledge over the input distributions. In realistic scenarios, such as online auctions, or allocation problems in general, this assumption fails to hold, and this motivates using the ``limited information" regime \citep{azar}. In particular, there will be a sample set $\mathcal{S}$ composed of $k$ samples coming from some of the distributions $F_1, \dots, F_n$, and a set $n$ of real online values $\mathcal{R}$, each one coming from its respective distribution. 
\begin{definition}\label{samples}
For distributions $F_1, \dots, F_n$, with $X_i \sim F_i$ and $S_j \sim F_\ell$, let
\begin{align*}
    \mathcal{S} &:= \{S_1, \dots, S_k\}\\
    \mathcal{R} &:= \{X_1, \dots, X_n\}
\end{align*}
be the sample and real sets respectively, with $k \in \mathbb{N}$.
\end{definition}

Based on the above notation, we now to introduce the notion of sample-based stopping rule, adapting the definition from \cite{correa}.

\begin{definition}
A $(k, n)$ stopping rule $\textbf{r}$ is an stopping rule that, given $k$ samples forming set $\mathcal{S}$, sets a stopping time $\tau \in [n]$ to accept value $X_\tau \in \mathcal{R}$.
\end{definition}

\begin{remark}
Note that any $(k, n)$ stopping rule $\textbf{r}$ can be reinterpreted as a $(0, k+n)$ stopping rule $\textbf{r}'$ that is constrained not to accept any of the first $k$ values.
\end{remark}

\subsection{Performance metrics}

There can be various potential ways of measuring online algorithmic performance, generally named as \emph{competitive ratios}. Indeed, we would like to assess how the stopping rule performs in expectation with respect to the optimum, given the randomness of the input system; at the same time, computing the expectation of the stopping rule and that of the optimum separately may give us a too pessimistic competitive ratio.

Oftentimes the easiest to compute, the $\RoE$, by the way it is defined, inevitably favours stopping rules running well on instances with large optimal value, insofar as small-valued instances do not play a significant role in the expectation computation; put another way, the $\RoE$ upholds stopping rules with good average-case performance in expectation. In contrast, the $\EoR$ evaluates the the stopping rule and the optimal value for all distribution instances distinctly and computes the expectation over them, thereby measuring algorithmic performance in a distributional average-case sense \cite{steger_eor}. As mentioned, our interest lies primarily in the following four:

\begin{definition}
For $X_1 \sim F_1, \dots, X_n \sim F_n$, let us define the following performance metrics:\footnote{In the case of prophet secretaries, the values will be arriving in random (and not adversarial) order.}
\begin{alignat}{2}
& \textbf{Ratio of Expectations}   \qquad && \RoE := \frac{\E\left[X_\tau\right]}{\E\left[\max_{i \in [n]}{X_i}\right]}\\
& \textbf{Expectation of Ratio}   \qquad && \EoR := \E\left[\frac{X_\tau}{\max_{i \in [n]}{X_i}}\right]\\
& \textbf{Expectation of Inverse Ratio}   \qquad && \EoIR := \E\left[\frac{\max_{i \in [n]}{X_i}}{X_\tau}\right]\\
& \textbf{Probability of selecting the maximum}   \qquad \qquad \qquad \qquad && \PbM := \Pr\left[X_\tau = \max_{i \in [n]}{X_i} \right]
\end{alignat}
Here, the expectation is taken over the distributions and possibly over the randomness of the stopping rule.
\end{definition}

\subsection{Classical Results}

Before introducing and proving the classical results in the space of optimal stopping, we begin by defining some families of stopping rules which will be of particular use throughout the rest of the paper.

\begin{definition}[Fixed Waiting Stopping Rules]\label{fixwait}
A stopping rule is said to be fixed waiting if after setting a number $T \in [n]$ appropriately, it rejects the first $T$ arrivals and picks the first subsequent realization that exceeds the maximum among the first $T$ values.
\end{definition}

The prophet variant of the same stopping rule can be outlined as follows.

\begin{definition}[Fixed Threshold Stopping Rules]\label{fixthresh}
A stopping rule is said to be fixed threshold if set a threshold $T \geq 0$ appropriately, it picks the first realization $X_\tau > T$.
\end{definition}

A more general stopping rule is one where the threshold is not unique and set a priori, but where the threshold changes based on the information seen so far and how much time is left before the end of the arrival process.

\begin{definition}[Adaptive Threshold Stopping Rules]\label{adapthresh}
A stopping rule is said to be adaptive threshold if, at each time step $i$
\begin{itemize}
    \item it sets a threshold $\sigma_i \geq 0$ depending on the values seen so far, the time step $i$, and the distributions (or samples in the case of unknown distributions).
    \item It picks $X_i > \sigma_i$, otherwise it rejects it.\\
\end{itemize}
\end{definition}

\noindent \emph{\textbf{Secretary.}}
\begin{theorem}[$1/e$ is optimal \citep{ferguson}]
For any collection of values $X_1, \dots, X_n$, there exists a stopping rule $\textbf{r}$ such that 
\begin{align}
    \Pr\left[X_\tau = \max_{i \in [n]}{X_i} \right] = \frac{1}{e}
\end{align}
Moreover, this stopping rule is fixed waiting.
\end{theorem}

\begin{proof}
We will start by proving that we can restrict our attention to the family of stopping rules of the fixed waiting form (as per Definition \ref{fixwait}): reject the first $r$ arrivals, and accept the first subsequent value exceeding the maximum among the first $r$ arrivals. We can immediately discard all cases where the $r^{\text{th}}$ arrival is not the maximum so far, given that picking such a value would make us lose certainly. Indeed, suppose we are at step $r \in [n]$, and consider the probability that the $r^{\text{th}}$ arrival is the maximum overall conditioned on the $r^{\text{th}}$ arrival being the maximum so far. 

Since the elements are shuffled uniformly at random, the probability that the highest value happens within the first $r$ arrivals is $r/n$. Given that we are conditioning on $X_{\pi_r}$ being the maximum so far, the above conditional probability is also equal to $r/n$. We notice that such a probability is an increasing function of $r$, and therefore, an optimal strategy that is willing to accept the maximum so far, should also be willing to accept a later maximum so far, which yields the strategy above.

Let us now denote by $p_r$ the winning probability for an arbitrary $r$, that is the probability we select the maximum by refusing $X_{\pi_1}, \dots, X_{\pi_{r}}$ and selecting the first subsequent value exceeding $\max_{j \in [r]}{X_{\pi_{j}}}$. We can write such a probability as
\begin{align*}
    p_r &= \sum_{i=1}^{n}{\Pr\left[X_\tau = X_{\pi_i} \ \wedge \ X_{\pi_i} = \max_{j \in [n]}{X_j}\right]}\\
    &= \sum_{i=1}^{n}{\Pr\left[X_\tau = X_{\pi_i} \given X_{\pi_i} = \max_{j \in [n]}{X_j}\right] \cdot \Pr\left[X_{\pi_i} = \max_{j \in [n]}{X_j}\right]}
\end{align*}

Suppose without loss of generality that the maximum occurs at index $i+1$, i.e. $X_{\pi_{i+1}} = \max_{j \in [n]}{X_j}$. Our stopping rule will not select the maximum unless $i \geq r$ and the maximum among the first $r$ arrivals is the same as the maximum among the first $i$, as otherwise we would pick the maximal value at an index between indices $\pi_i$ and $\pi_r$, and miss the true overall maximum. This event occurs with probability $r/i$, since it is the probability that the maximum of $i$ randomly shuffled values lands in the first $r$ of them. Formally, 
\begin{align*}
    \Pr\left[X_{\pi_i} = \max_{j \in [r]}{X_{\pi_j}} \given X_{\pi_i} = \max_{j \in [n]}{X_j}\right] = \frac{r}{i}
\end{align*}

Recalling that our stopping rule rejects the first $r$ values, we can rewrite the above expression for $p_r$ as
\begin{align*}
    p_r &= \sum_{i=r}^{n-1}{\Pr\left[X_{\pi_i} = \max_{j \in [r]}{X_{\pi_j}} \given X_{\pi_i} = \max_{j \in [n]}{X_j}\right] \cdot \frac{1}{n}} \\
    &= \frac{r}{n}\sum_{i=r}^{n-1}{\frac{1}{i}}\\
\end{align*}

We would now like to find the optimal $r$ for which $p_r$ is maximized. To this end, let us compute the following limit, noticing that the above sum can be written as an approximation of a Riemann integral. In particular, let $u = \lim_{n \rightarrow \infty}{r/n}$ and $w = \lim_{n \rightarrow \infty}{i/n}$. Then, 
\begin{align*}
    p_r = \lim_{n \rightarrow \infty}{\frac{r}{n}\sum_{i=r}^{n-1}{\frac{n}{i}\cdot\frac{1}{n}}} = u \cdot \int_{u}^{1}{\frac{1}{w}dw} = -u\ln u
\end{align*}
The above expression is maximized at $u = 1/e$ and the optimal $p_r = 1/e$. Hence,
\begin{align*}
    \Pr\left[X_\tau = \max_{i \in [n]}{X_i} \right] = \frac{1}{e}
\end{align*}

In essence, the optimal stopping rule reads: reject the first $n/e$ arrivals, and accept the first subsequent value exceeding the maximum among the first $n/e$ arrivals.
\end{proof}

\noindent \emph{\textbf{Prophet.}}

\begin{theorem}[$\RoE$ Lower Bound \cite{weinberg}]\label{roe-lb}
There exists a stopping rule that achieves a constant approximation to the $\RoE$.
\begin{align}
    \RoE := \frac{\E\left[X_\tau\right]}{\E\left[\max_{i \in [n]}{X_i}\right]} \geq \frac{1}{2}
\end{align}
Moreover, this stopping rule is fixed threshold.
\end{theorem}
\begin{proof}
We consider a simple fixed threshold stopping rule which sets $T := \mathbb{E}[\max_{i \in [n]}{X_i}]/2$. For notational simplicity, let $p := \Pr\left[\max_{i \in [n]}{X_i} > T\right]$, then, with probability $1-p$, the stopping rule rejects all arrivals and, thus, with probability at least $1-p$ it will have rejected all $X_1, \dots, X_{i-1}$. This means that for any $x > T$, the probability that the stopping rule accepts $X_i$ and $X_i > x$ is 
\begin{align*}
    \Pr[X_\tau = X_i \ \wedge \ X_i > x] \geq (1-p)\cdot\Pr[X_i > x]
\end{align*}

Since the event of accepting $X_i$ is disjoint from the event of accepting a different $X_j$, we get that the probability that the value we accept is above $x$ is 
\begin{align*}
    \Pr\left[X_\tau > x\right] \geq (1-p)\cdot\sum_{i =1}^{n}{\Pr[X_i > x]} \geq (1-p)\cdot\Pr[\max_{i \in [n]}{X_i} > x]
\end{align*}
where the last inequality follows directly from the union bound. Note that $\mathbb{E}[\max_{i \in [n]}{X_i}] = 2T$, and can be decomposed as follows
\begin{align*}
   \mathbb{E}[\max_{i \in [n]}{X_i}] = \int_0^T{\Pr[\max_{i \in [n]}{X_i} > x]} + \int_T^\infty{\Pr[\max_{i \in [n]}{X_i} > x]} = 2T
\end{align*}
The first integral must be at most $T$, and hence the second must be at least $T$. We can therefore write the following:
\begin{align*}
    \mathbb{E}[X_\tau] &= \int_0^T{\Pr[X_\tau > x]} + \int_T^\infty{\Pr[X_\tau > x]}\\
    &\geq pT + (1-p)\cdot\int_T^\infty{\Pr[\max_{i \in [n]}{X_i} > x]}\\
    &\geq pT + (1-p)T = T \\
    &= \frac{\mathbb{E}[\max_{i \in [n]}{X_i}]}{2}
\end{align*}
The claim thus follows.
\end{proof}

One may wonder whether more powerful stopping rules, such as adaptive threshold ones (Definition \ref{adapthresh}), yield higher $\RoE$. Below, we reprove a classical result that answers the above question in the negative, establishing that $1/2$ is a tight bound for $\RoE$.

\begin{observation}[$\RoE$ Upper Bound]\label{roe-ub}
There exists an instance of distributions $F_1, \dots, F_n$ such that $\RoE \leq 1/2$.
\end{observation}
\begin{proof}
Consider the following instance: $X_1 = 1$ deterministically and $X_2 = 0$ with probability $1 - \epsilon$, $X_2 = 1/\epsilon$ with probability $\epsilon$. We know that
\begin{align*}
    \mathbb{E}[\max\{X_1, X_2\}] = \frac{1}{\epsilon} \cdot \epsilon + 1 \cdot (1 - \epsilon) = 2 -\epsilon
\end{align*}
Any stopping rule cannot do better than $1$ in that if it accepts $X_1$ it will get $1$ deterministically, otherwise it accepts $X_2$ and gets $1$ in expectation. Therefore,
\begin{align*}
    \RoE := \frac{\E\left[X_\tau\right]}{\E\left[\max_{i \in [n]}{X_i}\right]} \leq \frac{1}{2-\epsilon}
\end{align*}
This concludes the proof of the observation, as $\epsilon$ is arbitrarily close to zero.
\end{proof}

==> sections/eoir.tex <==
\section{Reduction: from the $\EoR$ to best-choice prophet inequality}\label{reduction}

In this section, we will show that any stopping rule maximizing the expectation of ratio, also maximizes the probability of selecting the maximum in the online sequence, and vice versa. We do so by means of a reduction from any arbitrary distribution to a distribution where not picking the maximum is equivalent to having a zero approximation to the optimal value. For the case of I.I.D. random variables, we further show that the problem is equivalent to maximizing the probability of selecting the maximum for $X_1, \dots, X_n \stackrel{\text{IID}}{\sim} \text{Uniform}([0,1])$.

\begin{theorem}\label{reduction}
For a single choice online stopping problem and independent but non-identically distributed variables $X_1, \dots, X_n$, 
\begin{align*}
    \EoR \leq \PbM + o(1)
\end{align*}
In addition, for the case of independent and identically distributed random variables $X_1, \dots, X_n \stackrel{\text{IID}}{\sim} F$, we lose no generality by assuming that $F = \text{Uniform}([0,1])$.
\end{theorem}
\begin{proof}
We will prove the reduction by showing that for an stopping rule $\textbf{r}$, the $\EoR$ is equal to the probability of selecting the maximum in the online sequence $X_1, \dots, X_n$, up to vanishing small terms. Without loss of generality, let us assume that the support of each $F_i$ is an arbitrarily large discrete space, and denote it by $\text{support}(F_i)$.\footnote{Intuitively, if a large number of discrete values ``tends" towards a continuous support, so that we do not need to worry about continuous distributions.} Again not losing generality, we can assume that each of the values in the support is of the form $M^t$, for $t \in \mathbb{N}_0$, where $M$ as an arbitrarily large constant. Indeed, even if $M$ is the same constant, we choose it so that the gap between two consecutive values in the support is arbitrarily large and their ratio is arbitrarily close to $0$. Moreover, since the support of each $F_i$ has elements of the form $M^t$, taking the union over all of them lets us handle the cases of vastly different supports. Formally, let us now consider set $S$ defined as 
\begin{align*}
    S := \bigcup_{i \in [n]}{\text{support}(F_i)} = \left\{M^t \ | \ t \in \mathbb{N}_0 \right\} 
\end{align*}

Suppose that $\max_{i \in [n]}{X_i} = M^t$ and $\textbf{r}$ selects it with probability $p$. We note that for any $s < t$, the ratio is at most $1/M \in o(1)$. By definition of $p$,
\begin{align*}
    \EoR &= \E\left[\frac{X_\tau}{\max_{i \in [n]}{X_i}}\right] \leq p + (1-p) \cdot M^{-1} \\
    &= p + o(1) \\
    &= \Pr\left[X_\tau = \max_{i \in [n]}{X_i}\right] + o(1)
\end{align*}

For the case of I.I.D. random variables, we know that the support $S = \text{support}(F)$ is composed of elements in the form $M^b$, for some $b \in [n]$. For a known distribution from which $X_i$'s are drawn independently, the maximum over $X_i$'s still remains the maximum under all monotonic transformations, i.e., for all monotonic functions $\phi$, we have that
\begin{align*}
    Y = \max_{i \in [n]}{X_i} \Rightarrow \phi(Y) = \max_{i \in [n]}{\phi(X_i)}
\end{align*}

Therefore, we can assume that $F$ is uniform over its support with probability $\epsilon$, emphasizing the support must be composed of $1/\epsilon$ elements in order for this to be a (uniform) distribution, namely $S = \{1, M, \dots, M^{1/\epsilon - 1}\}$.\footnote{Note that we need to have that $M \rightarrow \infty$ faster than $\epsilon \rightarrow 0$.} Let us now scale the support dividing each element by $M^{1/\epsilon - 1}$, so that it is contained in the $[0,1]$ interval, thus obtaining $\tilde{S} = \{M^{-(1/\epsilon - 1)}, \dots, 1\}$. As $\epsilon \rightarrow 0$, the size of the support tends to infinity and the interval becomes $[0,1]$.
\end{proof}
\begin{remark}
The above theorem provides a reduction from the $\EoR$ to the $\PbM$. For the other direction, note that by definition we have
\begin{align*}
    \EoR \geq \PbM \cdot 1 + (1 - \PbM)\cdot\eta \geq \PbM
\end{align*}
for some $\eta < 1$.
\end{remark}

==> sections/ocrs.tex <==
\subsection{An OCRS Competitive Algorithm}
The idea behind our algorithm is based on defining a ``superstar'' to be the elements with value greater than $T$, which is the threshold set so that the maximum element is above it with probability $\gamma=1/2$. We distinguish  between two cases, (1) where selecting superstars is sufficient to get a good $\EoR$. In this case we ignore the multi-choice nature of the problem and we try to catch the superstar (that will be unique with probability of $1/4$). Else (2), we assume that no ``superstar'' arrives (with probability $1/2$), then run an Online Contention Resolution Scheme (OCRS) on the conditioned instance with no ``superstar'' element. In this case, we get that the performance of $\OPT$ is well concentrated, which is the key ingredient of our novel proof. 

In essence, a greedy OCRS, formally described in Definition ~\ref{ocrs-def}, can be outlined as follows: let $x_e := \Pr\left[w_e > \tau_e\right]$ be the probability of an element being \emph{active} for some thresholds $\tau_e > 0$, and consider the random set of \emph{active} elements be $R(\bx) := \left\{e \in E : w_e > \tau_e\right\}$. Since elements of $R(\bx)$ are revealed one by one, the algorithm's goal is to select a feasible subset of active elements such that it maximizes the expected overall weight. To this end, an OCRS selects each feasible element independently from the others with probability at least $\beta x_e$, i.e. $\Pr\left[e \in \ALG(\bw)\right] \geq \beta x_e$. This would in turn imply that $\E\left[\bw(\ALG(\bw))\right] \geq \beta \E\left[f(\bw)\right]$.

\subsubsection{Description}

\begin{definition}
For a finite ground set $E$ and a downward-closed family of feasibility constraints $\cF$, let $P_{\cF} \in [0, 1]^{|E|}$ be the convex hull of all its characteristic vectors, i.e.
\begin{align*}
    P_\cF = \text{conv}\left(\left\{\bone_{J} : J \in \cF\right\}\right).
\end{align*}
\end{definition}

\begin{definition}
A polytope $P \subseteq[0,1]^{|E|}$ is a relaxation of $P_\cF$ if $P \cap \{0, 1\}^{|E|} = P_\cF \cap \{0, 1\}^{|E|}$.
\end{definition}

\begin{definition}[Greedy Online Contention Resolution Schemes \cite{feldman-ocrs}]\label{ocrs-def}
Let elements $e \in E$ be revealed one by one in a fixed adversarial order, and let $\beta \in [0,1]$. An online selection algorithm $\ALG$ is called a $\beta$-selectable greedy OCRS if, for all $\bx \in P$, it defines a subfamily of feasibility constraints $\cF_{\bx}$, and, at every element arrival, it selects element $e \in E$ such that
\begin{align*}
    \Pr\left[J \cup \{e\} \in \cF_{\bx} \quad \forall J \subseteq R(\bx), J \in \cF_{\bx}\right] \geq \beta, \ \forall e \in E.
\end{align*}
A greedy OCRSs is called randomized if the choice of $\cF_{\bx}$ is itself randomized, and deterministic if it is fixed. Note that the deterministic version of a greedy OCRS has the above probability running over the randomness in $R(\bx)$ only, whilst the randomized one will additionally have the above probability running over $\cF_{\bx}$ randomness.
\end{definition}

In the proceedings, we use a specific kind of randomized greedy OCRS, which we will refer to as $(\beta, \bp)$-independent randomized greedy OCRS (or $(\beta, \bp)$-iOCRS in short). 
\begin{definition}[$(\beta, \bp)$-Independent Randomized Greedy OCRS]
Let us consider a downward-closed feasibility constraints family $\cF$, let $\beta \in [0,1]$ and let $\bp \in [0,1]^{|E|}$. A $(\beta, \bp)$-independent randomized greedy OCRS is a randomized greedy OCRS where the subfamily of feasibility constraints $\cF_{\bx}$ is constructed by tossing $|E|$ independent coins with probability vector $\bp$, obtaining a random set $S_{\bp}(\bx)$, and intersecting with all $J \in \cF$. Formally,
\begin{align*}
    \cF_{\bx} := \left\{S_{\bp}(\bx) \cap J: J \in \cF\right\}.
\end{align*}
Note that $\cF_{\bx}$ is a well-defined family since it is also downward-closed.
\end{definition}

Algorithmically, any $(\beta, \bp)$-iOCRS can be described as a procedure that selects element $e$ if the following three conditions occur jointly:
\begin{enumerate}
    \item Feasibility: $e$ is feasible.
    \item Activity: $e$ is active, in which case $w_e > \tau_e$.
    \item Coin flip: we toss a $\bp$ coin, and consider all the heads.
\end{enumerate}
Therefore, if we denote by $\bone_{e \in \ALG(\bw)}$ the random variable indicating whether element $e$ has been selected by the algorithm, we could also write it as a product of three indicators 
\begin{align*}
    \bone_{e \in \ALG(\bw)} = \bone_{e \text{ is feasible}}\bone_{w_e > \tau_e}\bone_{\text{coin}_e}.
\end{align*}

\begin{remark}\label{ocrs-feasibility}
Any $(\beta, \bp)$-iOCRS has $\Pr\left[e \text{ is feasible}\right] \geq \beta$, for all $e \in E$.
\end{remark}

\begin{observation}
Let us observe that
\begin{enumerate}
    \item Any $\beta$-selectable deterministic greedy OCRS is a special case of a $(\beta, \bp)$-iOCRS, with $\bp \in \{0,1\}^{|E|}$.
    \item The OCRS used for matching in general graphs with edge arrival by \citet{ezra} is also a special case of a $(\beta, \bp)$-iOCRS, with $p_e = \frac{\beta}{\Pr\left[e \text{ is feasible}\right]}$.
\end{enumerate}
\end{observation}

\RestyleAlgo{ruled}

\begin{algorithm}
\caption{$\EoR$-OCRS}\label{ocrs}
\KwData{Ground set $E$, distributions $D_e$, feasibility family $\cF$}
\KwResult{Subset $\ALG(\bw) \subseteq E$ such that $\ALG(\bw) \in \cF$}
$\ALG(\bw) \gets \emptyset$\;
\eIf{$\E\left[f(\overline{\bw})\right] \leq cT$}
{
    Select first element $e \in E$ such that $w_e \geq T$\;
    $\ALG(\bw) \gets \ALG(\bw) \cup \{e\}$\;
}{
    $\ALG(\bw) \gets \beta \text{-OCRS}(\bw)$\;
}
\end{algorithm}


\subsubsection{Analysis} 
In the proceedings, we stress that each expectation runs over the randomness coming from the input weights, name it $\bW$, and the randomness coming from the algorithm, say $\bA$, and from the offline optimum, say $\bO$.

\begin{definition}\label{events}
Let us define the following events.
\begin{enumerate}
    \item ``No superstar'': $\cE_0 := \left\{\forall e \in E: w_e \leq T\right\}$.
    \item ``Exactly one superstar'': $\cE_1 := \left\{\exists ! e \in E: w_e > T\right\}$,
\end{enumerate}
where the symbol ``$\exists !$'' signifies the existence of a unique such element.
\end{definition}

\begin{claim}[Adapted from Theorem 1 in \cite{esfandiari}]\label{gamma-lemma}
For any set of distributions $\{D_e\}_{e \in E}$,
\begin{align*}
    \Pr\left[\cE_0\right] &\geq \gamma,\\
    \Pr\left[\cE_1\right] &\geq \gamma \log\left(\frac{1}{\gamma}\right).
\end{align*}
\end{claim}

\begin{theorem}\label{ocrs-analysis}
Algorithm ~\ref{ocrs} produces a solution set $\ALG(\bw)$ such that
\begin{align}
    \E\left[\frac{\bw(\ALG(\bw))}{f(\bw)}\right] \geq O(\beta).
\end{align}
Moreover, since the analysis of Algorithm ~\ref{ocrs} hinges on a reduction to a $\beta$-OCRS, it is tight in the sense that we cannot achieve an expected competitive ratio larger than $\beta$. Nevertheless, it might be possible to design another algorithm achieving an expected competitive ratio larger than $\beta$ for specific feasibility constraints, although there is no better $\beta$-OCRS.
\end{theorem}

We divide the proof into two cases, i.e. cases where the subset of elements selected by $\OPT^\prime$ has a bounded weight in expectation as opposed to when it has a large weight. To be precise let us have the following case distinction.

\begin{lemma}\label{case1}
If $\E\left[f(\overline{\bw})\right] \leq cT$, Algorithm ~\ref{ocrs} produces a solution set $\ALG(\bw)$ such that
\begin{align}
    \E\left[\frac{\bw(\ALG(\bw))}{f(\bw)}\right] \geq \frac{\gamma \log\left(1/\gamma\right)}{c+1}.
\end{align}
\end{lemma}
\begin{proof}
In this scenario, we know that the OCRS competitive Algorithm ~\ref{ocrs} will select the first element $e \in E$ such that $w_e \geq T$. It may so happen that no such element exists in which case the OCRS algorithm gets a contribution to the $\EoR$ of $0$. On the other hand, by Claim ~\ref{gamma-lemma}, $\Pr\left[\cE_1\right] \geq \gamma \log\left(1/\gamma\right)$. Then, conditioned on this event happening, Algorithm ~\ref{ocrs} surely (with probability $1$) gets such an element and we have
\begin{align*}
    \frac{\bw(\ALG(\bw))}{f(\bw)} &\geq \frac{w_e}{w_e + f(\overline{\bw})}\\
    &\geq \frac{T}{T + f(\overline{\bw})}.
\end{align*}
Here, the first inequality follows from Claim ~\ref{opts}, and the second by observing that since $w_e > T$, the worst possible case for the ratio is when both the $w_e$ in the numerator and the denominator are equal to $T$. Hence, by the above and the law of total expectation
\begin{align*}
    \E\left[\frac{\bw(\ALG(\bw))}{f(\bw)}\right] &\geq \E\left[\frac{\bw(\ALG(\bw))}{f(\bw)} \given \cE_1\right] \cdot \Pr\left[\cE_1\right]\\
    &\geq \E\left[\frac{T}{T + f(\overline{\bw})}\right] \cdot \gamma \log\left(1/\gamma\right)\\
    &\geq \frac{T}{T + \E\left[f(\overline{\bw})\right]} \cdot \gamma \log\left(1/\gamma\right)\geq \frac{\gamma \log\left(1/\gamma\right)}{c+1}.
\end{align*}
The second inequality follows from noticing that conditioning the realization of $\bw$ on $\cE_1$ is equivalent from drawing weights from distributions $\overline{D}_e$'s, i.e. obtaining $\overline{\bw}$. The third inequality follows directly from Claim ~\ref{jensen}, whilst the last inequality derives from the assumption that $\E\left[f(\overline{\bw})\right] \leq cT$. The statement follows.
\end{proof}

\begin{lemma}\label{case2}
If $\E\left[f(\overline{\bw})\right] > cT$, Algorithm ~\ref{ocrs} produces a solution set $\ALG(\bw)$ such that
\begin{align}
    \E\left[\frac{\bw(\ALG(\bw))}{f(\bw)}\right] \geq \gamma \cdot \frac{\lambda-1}{\lambda} \cdot \frac{\nu-1}{\nu} \cdot \frac{\beta}{\delta}
\end{align}
\end{lemma}
\begin{proof}
In this setting, Algorithm ~\ref{ocrs} selects element $e \in E$ if $w_e > \tau_e$ (which happens with probability $y_t$), if it is feasible and it is active according to the $\beta$-OCRS algorithm. We conservatively assume that the contribution to the expected competitive ratio will be $0$, should there exist some element whose weight exceeds $T$. By Claim ~\ref{gamma-lemma}, $\Pr\left[\cE_0\right] \geq \gamma$: we omit the conditioning on this event in the derivation below for ease of notation. This implies that the right summand of Claim ~\ref{opts} will be $0$, and we have that
\begin{align*}
        \E\left[\frac{\bw(\ALG(\bw))}{f(\bw)}\right] &\geq \E\left[\frac{\bw(\ALG(\bw))}{f(\bw)} \given \cE_0\right] \cdot \Pr\left[\cE_0\right] \\
        &= \gamma \sum_{e \in E}{\E\left[\frac{w_e \cdot \bone_{e \in \ALG(\bw)}}{f(\bw)} \given \cE_0\right]} \\
        &= \gamma \sum_{e \in E}{\E\left[\frac{w_e \cdot \bone_{\text{coin}_e}}{f(\bw)} \given e \text{ is feasible}, w_e > \tau_e, \cE_0 \right]} \cdot \Pr\left[e \text{ is feasible}, w_e > \tau_e, \cE_0\right].
\end{align*}
The last equality follows from the fact that $\bone_{e \in \ALG(\bw)} = \bone_{e \text{ is feasible}}\bone_{w_e > \tau_e}\bone_{\text{coin}_e}$. Moreover, noting that $w_e$ and $f(\bw)$ are correlated, we now construct a new set in a way that its weight is uncorrelated to that of element $e$. Fixed a realization of weights $\bw$, we replace the the weight $w_e$ of element $e$ with $T$: this is exactly $\OPT(\widetilde{\bw}_{-e})$. Note that $f\left(\widetilde{\bw}_{-e}\right)$ is now completely independent from $w_e$ and, by monotonicity in Claim ~\ref{addw}, $f(\bw) \leq f\left(\widetilde{\bw}_{-e}\right)$. We denote with $W := \E\left[f(\bw)\right]$ and lower bound the above sum by
\begin{align*}
    &\geq \sum_{e \in E}{\E\left[\frac{w_e \cdot \bone_{\text{coin}_e}}{f\left(\widetilde{\bw}_{-e}\right)} \given e \text{ is feasible}, w_e > \tau_e, \cE_0 \right]} \cdot \Pr\left[e \text{ is feasible}, w_e > \tau_e, \cE_0 \right]&\\
    &\geq \sum_{e \in E}{\E\left[\frac{w_e \cdot \bone_{\text{coin}_e}}{f\left(\widetilde{\bw}_{-e}\right)} \given e \text{ is feasible}, w_e > \tau_e, f\left(\widetilde{\bw}_{-e}\right) \leq \delta W, \cE_0 \right]&}\\
    &\quad\qquad \cdot \Pr\left[e \text{ is feasible}, w_e > \tau_e, \cE_0 \right] \cdot \Pr\left[f\left(\widetilde{\bw}_{-e}\right) \leq \delta W \given e \text{ is feasible}, w_e > \tau_e, \cE_0 \right].&
\end{align*}
We now continue the proof of the theorem by assuming Claim ~\ref{goodset}, stated below and proven at the end of this section.
\begin{restatable*}{claim}{goodset}\label{goodset}
For $\delta, \lambda, \nu > 1$ appropriately defined constants, and for all $e \in E$, we have
\begin{align*}
    \Pr\left[f\left(\widetilde{\bw}_{-e}\right) \leq \delta W \given e \text{ is feasible}, w_e > \tau_e, \cE_0 \right] \geq \frac{\lambda - 1}{\lambda} \cdot \frac{\nu - 1}{\nu}.
\end{align*}
\end{restatable*}

Assuming the above claim holds, the above is lower bounded by
\begin{align*}
    &\geq \frac{\lambda-1}{\lambda} \cdot \frac{\nu - 1}{\nu} \cdot \frac{1}{\delta W} \\
    &\qquad\qquad \cdot \sum_{e \in E}{\E\left[w_e \cdot \bone_{\text{coin}_e} \given e \text{ is feasible}, w_e > \tau_e, \cE_0 \right]} \cdot \Pr\left[e \text{ is feasible}, w_e > \tau_e, \cE_0 \right]\\
    &\geq \frac{\lambda-1}{\lambda} \cdot \frac{\nu-1}{\nu} \cdot \frac{\beta}{\delta}.
\end{align*}

The last inequality follows from the fact that the sum is exactly what OCRS algorithm gets. In conclusion, we get a contribution to the expected competitive ratio of
\begin{align*}
    \gamma \cdot \frac{\lambda-1}{\lambda} \cdot \frac{\nu-1}{\nu} \cdot \frac{\beta}{\delta}.
\end{align*}
This concludes the proof.
\end{proof}

\begin{proof}[Proof of Theorem ~\ref{ocrs-analysis}]
Let us first note that Algorithm ~\ref{ocrs} will guarantee the minimum between the expected competitive ratios of Lemmata ~\ref{case1}, ~\ref{case2}. Namely, we need to solve following nonlinear constrained optimization problem:
\begin{align*}
    &\min\left\{\frac{\gamma \log\left(1/\gamma\right)}{c+1}, \gamma \cdot \frac{\lambda-1}{\lambda} \cdot \frac{\nu-1}{\nu} \cdot \frac{\beta}{\delta}\right\} \quad &\triangleleft \text{ Lemmata ~\ref{case1}, ~\ref{case2}}\\
    &\text{s.t. } \enspace \delta = 6\lambda \\
    &\qquad c = 10\log\left(1 + \frac{\nu}{\beta}\right) &\\
    &\qquad 0 < \gamma < 1 &\\
    &\qquad \lambda, \nu > 1. &
\end{align*}
Observe that $\beta$ is the only parameter we do not control, insofar as it depends on the feasibility structure we are dealing with. Let us choose the following constants: $\gamma = 1/2, \lambda = 2, \nu = 2$, to get $\delta = 12$ and $c = 10\log\left(1 + \frac{\nu}{\beta}\right)$. All in all, we get that the expected competitive ratio is 
\begin{align*}
    \E\left[\frac{\bw(\ALG(\bw))}{f(\bw)}\right] \geq \min\left\{\frac{\log 2}{20\log\left(1 + \frac{2}{\beta}\right) + 2}, \frac{\beta}{96}\right\} = \frac{\beta}{96}.
\end{align*}
where the last equality always holds for any $\beta > 0$. Note that, in addition, parameters $\gamma < 1, (\lambda-1)/\lambda \leq 1, (\nu-1)/\nu \leq 1, \delta > 1$ (as $c$ would not influence the left hand side of the minimum expression), and they would not necessarily be feasible constants and would make us achieve at most a $\beta$ factor: this is just a marginal improvement with respect to our \emph{feasible} choice of parameters.
\end{proof}

We can now prove Claim ~\ref{goodset} needed for Lemma ~\ref{case2} of Theorem ~\ref{ocrs-analysis}.

\goodset
\begin{proof}
By the way $\OPT(\widetilde{\bw}_{-e})$ is defined, conditioning on $w_e > \tau_e$ is irrelevant for random variable $f\left(\widetilde{\bw}_{-e}\right)$, as the latter does not depend on the weight of $e$. Secondly, let us define the following random Boolean string $s$ encoding whether or not each element weight is above its threshold between element $1$ and $e$:
\begin{align*}
    s := \left\{\bone_{w_{e^\prime} > \tau_{e^\prime}} \mid e^\prime < e\right\}.
\end{align*}
Similarly, let $\cG$ be the set of ``good'' Boolean strings,
\begin{align*}
    \cG &:= \left\{b \in \{0,1\}^{e-1} \given \E\left[f\left(\widetilde{\bw}_{-e}\right) \mid s = b, \cE_0 \right] \leq \eta W\right\}.
\end{align*}
Hence, we can write
\begin{align*}
    \Pr&\left[f\left(\widetilde{\bw}_{-e}\right) \leq \delta W \mid e \text{ is feasible}, w_e > \tau_e, \cE_0 \right] \\
    &\geq \sum_{b \in \cG}{\Pr\left[f\left(\widetilde{\bw}_{-e}\right) \leq \delta W \mid s = b, e \text{ is feasible}, \cE_0 \right] \cdot \Pr[s = b \mid e \text{ is feasible}, \cE_0 ]}\\
    &= \sum_{b \in \cG}{\Pr\left[f\left(\widetilde{\bw}_{-e}\right) \leq \delta W \mid s = b, \cE_0 \right] \cdot \Pr[s = b \mid e \text{ is feasible}, \cE_0 ]}\\
    &\geq \frac{\lambda-1}{\lambda} \cdot \sum_{b \in \cG}{\Pr[s = b \mid e \text{ is feasible}, \cE_0 ]} = \frac{\lambda-1}{\lambda} \cdot \Pr[s \in \cG \mid e \text{ is feasible}, \cE_0 ].
\end{align*}
The equality follows from the fact that the algorithm would act the same once we condition on $S$ being a ``good'' fixed Boolean string $b$, and therefore $f\left(\widetilde{\bw}_{-e}\right)$ is independent of the random variable indicating that $e$ is feasible. The last inequality derives from the fact that, if $s = b$, for $b \in \cG$, then by Markov's inequality and letting $W_b := \E\left[f\left(\widetilde{\bw}_{-e}\right) \mid s = b, \cE_0 \right]$,
\begin{align*}
    \Pr\left[f\left(\widetilde{\bw}_{-e}\right) \leq \lambda\eta W \given s = b, \cE_0 \right] &\geq \Pr\left[f\left(\widetilde{\bw}_{-e}\right) \leq \lambda W_b \given s = b, \cE_0 \right] \geq 1 - \frac{1}{\lambda},
\end{align*}
so that $\delta=\lambda\eta$. What is left to be shown is that $\Pr[s \in \cG \mid e \text{ is feasible}, \cE_0]$ is also at least constant. We first show that the following holds:
\begin{claim}\label{opt-talagrand}
$\Pr\left[s \in \cG \mid \cE_0\right] \geq 1 - \beta/\nu$.
\end{claim}
\begin{proof}
Let us observe that understanding whether $S$ is a ``good'' string is equivalent to draw independent random weights $w_1, \dots, w_{|E|}$, construct the corresponding binary string $b(\bw)$, and see whether it is, in fact, ``good''. For ease of notation, let us define $W_{b(\bw)} := \E\left[f\left(\widetilde{\bw}_{-e}\right) \mid s = b(\bw), \cE_0 \right]$. Assume for contradiction that, with probability greater than $\beta/\nu$, $W_{b(\bw)} > \eta W$. Then, we get
\begin{align*}
    \Pr\left[f\left(\widetilde{\bw}_{-e}\right) > \frac{\eta}{2} W \mid \cE_0\right] &\geq \sum_{b \notin \cG}\Pr\left[f\left(\widetilde{\bw}_{-e}\right) > \frac{\eta}{2} W \given b(\bw) = b, \cE_0 \right] \cdot \Pr\left[b(\bw) = b \mid \cE_0 \right] \\
    &\geq \sum_{b \notin \cG}\Pr\left[f\left(\widetilde{\bw}_{-e}\right) > \frac{W_{b(\bw)}}{2} \given b(\bw) = b, \cE_0 \right] \cdot \Pr\left[b(\bw) = b \mid \cE_0 \right].
\end{align*}
We now apply Corollary ~\ref{blm-T} to lower bound the above expression. Indeed, blm inequality is applicable since $f$ is a self-bounding function. Thereby, we use the lower tail bound and choose $z := \frac{W_{b(\bw)}}{2T}$, 
\begin{align*}
    \Pr\left[f\left(\widetilde{\bw}_{-e}\right) > \frac{W_{b(\bw)}}{2} \given b(\bw) = b, \cE_0 \right] \geq 1 - e^{-\frac{c}{8}},
\end{align*}
which also follows from $W_{b(\bw)} \geq cT$. Then, we get
\begin{align*}
    \Pr\left[f\left(\widetilde{\bw}_{-e}\right) > \frac{\eta}{2} W \mid \cE_0\right] &\geq \left(1 - e^{-\frac{c}{8}}\right)\sum_{b \notin \cG}\Pr\left[b(\bw) = b \mid \cE_0 \right]\\
    &= \left(1 - e^{-\frac{c}{8}}\right)\Pr\left[b(\bw) \notin \cG \mid \cE_0 \right]\\
    &> \frac{\beta}{\nu} \left(1 - e^{-\frac{c}{8}}\right).
\end{align*}
On the other hand, however, we have that, by the 1-Lipschitz condition, $f\left(\widetilde{\bw}_{-e}\right) \leq f(\bw) + T$, and therefore, by taking expectations, we have
\begin{align*}
 W \geq \E\left[f\left(\widetilde{\bw}_{-e}\right) \mid \cE_0 \right] - T \geq \frac{1}{c}W + \left(1 - \frac{1}{c}\right)\E\left[f\left(\widetilde{\bw}_{-e}\right) \mid \cE_0 \right] - T \geq \left(1 - \frac{1}{c}\right)\E\left[f\left(\widetilde{\bw}_{-e}\right) \mid \cE_0 \right],
\end{align*}
where the last inequality follows again from $W > cT$. By the blm inequality in Corollary ~\ref{blm-T},
\begin{align*}
    \Pr\left[f\left(\widetilde{\bw}_{-e}\right) > \frac{\eta}{2}W \given \cE_0 \right] \leq \Pr\left[f\left(\widetilde{\bw}_{-e}\right) > \frac{\eta}{2}\left(1 - \frac{1}{c}\right) \E\left[f\left(\widetilde{\bw}_{-e}\right) \mid \cE_0 \right] \given \cE_0 \right] \leq e^{-\frac{c}{10}},
\end{align*}
which follows from $z := \frac{1}{T}\left(\frac{\eta}{2}\left(1 - \frac{1}{c}\right) - 1\right)\E\left[f\left(\widetilde{\bw}_{-e}\right) \mid \cE_0 \right] \geq c\left(\frac{\eta}{2}\left(1 - \frac{1}{c}\right) - 1\right) \geq \frac{c}{2}$, for $c \geq 2$ and $\eta = 6$. If we combine the above and choose $c = 10\log\left(1 + \frac{\nu}{\beta}\right)$, we obtain the following contradiction:
\begin{align*}
    \frac{e^{-\frac{c}{10}}}{1 - e^{-\frac{c}{8}}} \geq \frac{e^{-\frac{c}{10}}}{1 - e^{-\frac{c}{10}}} = \frac{\beta}{2\nu - \beta}> \frac{\beta}{\nu} \Longrightarrow \nu < \beta.
\end{align*}
This is impossible since $\beta \leq 1$ and $\nu > 1$ always. Hence, the claim follows.
\end{proof}

\noindent By the above, we can thus write
\begin{align*}
    1 - \frac{\beta}{\nu} &\leq \Pr\left[s \in \cG \mid \cE_0 \right] \\
    &= \Pr\left[s \in \cG \mid e \text{ is feasible}, \cE_0 \right] \cdot \Pr\left[e \text{ is feasible} \mid \cE_0 \right] \\
    &\quad + \Pr\left[s \in \cG \mid e \text{ is unfeasible}, \cE_0 \right] \cdot \Pr\left[e \text{ is unfeasible} \mid \cE_0 \right]&\\
    &\leq \Pr\left[s \in \cG \mid e \text{ is feasible}, \cE_0 \right] \cdot \Pr\left[e \text{ is feasible} \mid \cE_0 \right] + 1 - \Pr\left[e \text{ is feasible} \mid \cE_0 \right].&
\end{align*}
Rearranging,
\begin{align*}
    \Pr\left[s \in \cG \mid e \text{ is feasible}, \cE_0\right] \geq \frac{1 - \beta/\nu + \Pr\left[e \text{ is feasible} \mid \cE_0 \right] - 1}{\Pr\left[e \text{ is feasible} \mid \cE_0 \right]} \geq \frac{(1-1/\nu)\beta}{\beta} = 1 - \frac{1}{\nu}.
\end{align*}
where the last inequality follows from the OCRS guarantee to have element $e$ feasible with probability at least $\beta$ by Remark ~\ref{ocrs-feasibility}. All in all, 
\begin{align*}
    \Pr\left[f\left(\widetilde{\bw}_{-e}\right) \leq \delta W \given e \text{ is feasible}, w_e > \tau_e, \cE_0\right] \geq \frac{\lambda - 1}{\lambda} \cdot \frac{\nu - 1}{\nu},
\end{align*}
and the claim follows.
\end{proof}

==> sections/old.tex <==
\subsection{Extension to Single-sample}\label{app:ss} 
In this appendix, we discuss an extension of our results to the case of single sample settings. In our results and definitions, we assumed that the algorithm has  \emph{full knowledge} of the distributions from where the elements' weights are drawn. This is used to calculate the threshold $\tau$ in \Cref{eq:t} for a fixed $\gamma$ and perform the case distinction ``catch the superstar'' vs. ``run the combinatorial algorithm'' (see also \Cref{general,general-rev}). On the other hand, as mentioned in \Cref{relwork}, there has been significant effort towards designing prophet inequalities with provable guarantees when the decision-maker has only access to some samples from each distribution. We explain now how our result can be extended to single sample settings.
To do so, we first define equivalent definitions to those of \Cref{sec:model}.

Our objective is to design single-sample algorithms that maximize the expected ratio between what the online algorithm gets, and the weight of the offline optimum with full distributional knowledge. To measure our performance, given a downward-closed family $\cF$, an algorithm $\ALG$, and a product distribution $D$, we define
\begin{align*}
    \SEoR(\cF, \ALG, D) := \E\left[\frac{\bw(\ALG(\bw))}{f(\bw)}\right],
\end{align*}
where the expectation runs over the stochastic generation of the input, as well as the (possible) randomness of the algorithm.
Similarly, we define 
%given a downward-closed family $\cF$, a product distribution $D$
\begin{equation}
    \SEoR(\cF,\ALG) := \inf_{D} \SEoR(\cF, \ALG, D), \label{eq:SEORD}% \E\left[\frac{\bw(\ALG(\bw))}{f(\bw)}\right],
\end{equation}
and
\begin{equation}
    \SEoR(\cF):= \sup_{\ALG}  \SEoR(\cF,\ALG). \label{eq:SEORF} %\E\left[\frac{\bw(\ALG(\bw))}{f(\bw)}\right],
\end{equation}


We will compare our results to the standard objective of maximizing the ratio of expectations between the algorithm and the offline optimum. Accordingly, we denote
\begin{align*}
    \SRoE(\cF, \ALG, D) := \frac{\E\left[\bw(\ALG(\bw))\right]}
    {\E\left[{f(\bw)}\right]}.
\end{align*}

Analogously to Equations~\eqref{eq:SEORD},~and \eqref{eq:SEORF}, we define $\SRoE(\cF,\ALG)$ and  $\SRoE(\cF)$.

\begin{corollary}[Single-sample simulation]\label{cor:ss}
%Let $\EoR_{S}(\cF)$ and $\RoE_S(\cF$ denote the ratio of expectations and expectation of ratio, respectively, in the case of the  as defined in  but for single sample from each distribution $D_e$. 
If the product distribution $D$ is unknown, but the decision maker has access to a single sample from each distribution $D_e$, then for every downward-closed family of feasibility sets $\cF$, it holds that
\begin{align}
\emph{\SEoR}(\cF) \geq \frac{\emph{\SRoE}(\cF)}{96}.
\end{align}
%for the same choice of parameters as in \Cref{alg-analysis}.
\end{corollary}

\begin{proof}
Although we cannot compute the expected optimum of an instance and perform the case distinction, we can still flip a fair coin and run either of the two subroutines. We denote by $S = \{ s_e \mid e \in E \}$ the sample set, and by $O = \{ o_e \mid e \in E \}$ the online set.

For the ``catch the superstar'' case, 
we set $T = \max_{e \in E} s_e$ to be the threshold above which we accept in the online sequence. Observe that this algorithm selects the maximum only when the element with the largest weight is in the online set, and the element with the second largest weight (among the $2|E|$ weights in total) is in the sample set. It is not difficult to see that this happens with probability $1/4$ since the draws are independent (see also the principle of deferred decisions in~\citep[Section~3]{rubinstein}). Let $R = S \cup O$ and $r_1 > r_2 > \dots > r_{2|E|}$ denote the weights in $R$ sorted in decreasing order. Moreover, fixing a parameter $\gamma \in (0,1)$ as before, we define the threshold $\tau$ to be such that 
\begin{equation}
    \Pr\left[\tau \geq \max_{e \in E}{o_e}\right] = \gamma. 
\end{equation}
%and $e^* := \arg\max_{e \in H} w_e$.
 Considering the contribution only from the instances for which $W \leq c \cdot \tau$ for some $c>0$, and following the analysis of \Cref{newcase1}, we get

\begin{align*}
    \E\left[\frac{a(\bw)}{f(\bw)}\right] &\geq \Pr[\text{coin}] \cdot \Pr\left[ r_1 \in O \wedge r_2 \in S \right] \cdot  \E\left[\frac{a(\bw)}{f(\bw)} \given \cE_1\right] \cdot \Pr\left[\cE_1\right]  \\
    %\Pr[\text{coin}] \cdot \Pr\left[ w_{e^*} \in O \wedge \max_{e \neq e^*, e \in H} w_e \in S \right] \cdot  \E\left[\frac{a(\bw)}{f(\bw)} \given \cE_1\right] \cdot \Pr\left[\cE_1\right]  \\
    &\geq \frac{\gamma \log\left(1/\gamma\right)}{8(c+1)}.\\
\end{align*}
For the ``run the combinatorial algorithm'' case, we assume the existence of an algorithm $\AALG$ that, given a single sample from each distribution in the input, satisfies $\E\left[a_{\AALG}(\bw)  \mid \cE_0 \right]  \geq \alpha \cdot  \E\left[f(\bw) \mid  \cE_0\right]$. As long as $o_e \leq \tau$, we run the single sample algorithm $\AALG$; if $o_e>\tau$, we reject all remaining elements. Similar to the analysis with full knowledge of the distributions (see \Cref{newcase2}), we count the contribution of our algorithm only when the realized weights of all samples \emph{and} online values are bounded above by $\tau$ (observe that this happens independently for $S$ and $O$). Concretely, combining with \Cref{newcase2}, we have that
\begin{equation*}
        \E\left[\frac{a(\bw)}{f(\bw)}\right]  \geq \Pr[\text{coin}] \cdot \E\left[\frac{a(\bw)}{f(\bw)} \given \cE_0\right] \cdot \Pr\left[\cE_0\right] \cdot \Pr\left[\cE_0\right] \geq \frac{\gamma^2}{2\delta}\frac{k-\delta}{k}\alpha ,
\end{equation*}
which means that we lose a multiplicative factor of $\gamma/2$ compared to the full information case. 

The described algorithm, which flips a fair coin to decide which of the two cases to run, guarantees the minimum between the two expected competitive ratios. Choosing the parameters as in \Cref{alg-analysis}, we obtain 
\begin{align*}
    \SEoR = \min\left\{\frac{\frac{1}{16} \log 2}{\frac{8}{3} \log \frac{3}{\alpha} +1}, \frac{\alpha}{48}\right\} \geq \frac{\alpha}{96}.
\end{align*}
This concludes the proof.
\end{proof}
Note that the direction from $\SEoR$ to $\SRoE$ follows from similar arguments.






















\section{Old Proofs, Ideas, Facts}
{\color{red}
\subsection{A note on self-bounding functions}
Let us define $f(S)$ to be the function maximizing the sum of element weights subject to a downward-closed (packing) constraint, but only for elements $e \in S \subseteq E$ (e.g. max-weight matching for elements confined to $S$). Hence, $f: 2^E \rightarrow \mathbb{R}$, and
\begin{align*}
    f(S) := \max_{J \in \cF: J \subseteq S}{\sum_{e \in J}{w_e}}.
\end{align*}
We now proceed with two useful definitions: XOS (fractionally subadditive) functions and self-bounding functions. Our plan will be to prove that $f$ is XOS for all downward-closed constraints, show the the former is a subset of the latter, and point out to a strong concentration bound for self-bounding functions to demonstrate concentration for $f$ whenever $w_e \leq T$, for all $e \in E$. To this end, we use a standard scaling argument and assume all $w_e \leq 1$, without loss of generality.

\begin{definition}[Marginal Value \cite{vondrak}]
For a function $g: 2^E \rightarrow \mathbb{R}$, the marginal value of $e \in E$ with respect to $S \subseteq E$, is $g_S(e) :=  g(S \cup \{e\}) - g(S)$. $g$ is called $L$-Lipschitz, if its marginal values are bounded by $L$ in absolute value.
\end{definition}

{\color{blue} For a reference: \url{https://theory.stanford.edu/~jvondrak/data/submodular-chernoff.pdf}}

\begin{definition}[XOS (fractionally subadditive) functions]
A function $g: 2^E \rightarrow \mathbb{R}$ is said to be XOS (fractionally subadditive) if there exists a finite number of additive functions $\alpha_1, \dots, \alpha_r$ such that 
\begin{align*}
    g(S) = \max\{\alpha_1(S), \dots, \alpha_r(S)\}.
\end{align*}
An alternative definition is that, whenever, for all $e^\prime \in S$, $b_e \geq 0$ and $\sum_{e: e^\prime \in B_{e}}{b_e} \geq 1$, 
\begin{align*}
    g(S) \leq \sum_{e \in E}{b_e g(B_e)}.
\end{align*}
\end{definition}

\begin{claim}\label{xos}
$f$ is XOS.
\end{claim}
\begin{proof}
Let $\{J_1, \dots, J_r\}$ be the enumeration of all feasible sets for family of constraints $\cF$, and set $\alpha_i(S) := \sum_{e \in S \cap J_i}{w_e}$, for $i \in [r]$, $S \subseteq E$. Note that each of these functions can be written as an additive function insofar as 
\begin{align*}
    \alpha_i(S) = \sum_{e \in S}{w_e \bone[e \in J_i]},
\end{align*}
Since $f(S)$ is the value of the max-weight feasible set composed of elements in $S$ only, we get $f(S) = \max\{\alpha_1(S), \dots, \alpha_r(S)\}$.
\end{proof}

{\color{blue} For a reference: Proposition 4.1 in \url{https://arxiv.org/pdf/1610.00901.pdf}}

Before proceeding, it is important to stress that $f$ has been so far defined on sets, but the following definition is on a vector of weights on elements of such sets. In essence, the function will now be of the form $f: [0,1]^E \rightarrow \mathbb{R}$ as opposed to $f: 2^E \rightarrow \mathbb{R}$, and thus we need to show a construction mapping the set function to the value function on the continuous hypercube.

\begin{definition}[Self-bounding functions]
A function $g: [0,1]^E \rightarrow \mathbb{R}$ is said to be self-bounding if there exist functions $g_e: [0,1]^{E-1} \rightarrow \mathbb{R}$ such that, denoting by $\bw^{(e)} := (w_1, \dots, w_{e-1}, w_{e+1}, \dots, w_{|E|})$,
\begin{align*}
    &0 \leq g(\bw) - g_e(\bw^{(e)}) \leq 1,\\
    &\sum_{e \in E}{g(\bw) - g_e(\bw^{(e)})} \leq g(\bw).
\end{align*}
\end{definition}

\begin{theorem}[Boucheron-Lugosi-Massart Inequality \cite{bml}]\label{bml}
Let $\bw$ be a vector of independent random variables $w_1, \dots, w_{|E|}$ such that $\abs{w_e} \leq 1$, we have that for self-bounding functions $g: [0,1]^{|E|} \to \mathbb{R}$, and for any $\zeta > 0$,
\begin{align*}
    \Pr\left[g(\bw) \geq \E\left[g(\bw)\right] + \zeta \right] \leq e^{-\frac{\zeta^2}{2\E\left[g(\bw)\right] + 2\zeta/3}}.
\end{align*}
On the other hand, for $0 < \zeta \leq \E\left[g(\bw)\right]$,
\begin{align*}
    \Pr\left[g(\bw) \leq \E\left[g(\bw)\right] - \zeta \right] \leq e^{-\frac{\zeta^2}{2\E\left[g(\bw)\right]}}.
\end{align*}
\end{theorem}

\begin{corollary}\label{bml-T}
Let $\bw$ be a vector of independent random variables $w_1, \dots, w_{|E|}$ such that $\abs{w_e} \leq T$, we have that for $T$-self-bounding functions $g: [0,T]^{|E|} \to \mathbb{R}$, and for any $\zeta > 0$,
\begin{align*}
    \Pr\left[g(\bw) \geq \E\left[g(\bw)\right] + \zeta T \right] \leq e^{-\frac{\zeta^2}{2\E\left[g(\bw)\right] + 2\zeta/3}}.
\end{align*}
On the other hand, for $0 < \zeta \leq \E\left[g(\bw)\right]$,
\begin{align*}
    \Pr\left[g(\bw) \leq \E\left[g(\bw)\right] - \zeta T \right] \leq e^{-\frac{\zeta^2}{2\E\left[g(\bw)\right]}}.
\end{align*}
\end{corollary}

{\color{blue} For a reference: Theorem 6.12 in \url{https://www.hse.ru/data/2016/11/24/1113029206/Concentration\%20inequalities.pdf}}

Our last step is to show that all XOS functions are, in fact, self-bounding.

\begin{lemma}\label{xos-self}
Let $g: 2^{|E|} \to \mathbb{R}$ be an XOS function with marginal values in $[0,1]$. Then, $g: [0,1]^{|E|} \to \mathbb{R}$ is self-bounding.
\end{lemma}
\begin{proof}
Since $g$ is monotone, we can equivalently use for $\bw^{(e)} := (w_1, \dots, w_{e-1}, 0, w_{e+1}, \dots, w_{|E|})$, so that $g(\bw) - g_e(\bw^{(e)})$ is the marginal value of $e$ with respect to the set induced by the coordinates of $\bw^{(e)}$. Thus, $0 \leq g(\bw) - g_e(\bw^{(e)}) \leq 1$ is satisfied by assumption and the $1$-Lipschitz condition. 

We are now going to use the alternative definition of XOS function, namely the one motivating the name fractionally subadditive, and define $S := \{e \in E: w_e \neq 0\}$ while $B_e := S \setminus \{e\}$, $b_e := \frac{1}{|E|-1}$. Hereby, we have that $\sum_{e: e^\prime \in B_e}{b_e} = (|E|-1) \cdot \frac{1}{|E|-1} = 1$. Moreover, we abuse notation and write $g(\bw) = g(S)$, and $g_e(\bw^{(e)}) = g(B_e)$, so that, by definition of fractional subadditivity,
\begin{align*}
    g(\bw) = g(S) \leq \sum_{e \in E}{b_e g(B_e)} = \frac{1}{|E|-1}\sum_{e \in E}{g_e(\bw^{(e)})},
\end{align*}
which proves the second required condition for the self-bounding property. The lemma follows.
\end{proof}

{\color{blue} For a reference: \url{https://theory.stanford.edu/~jvondrak/data/submodular-chernoff.pdf}}

\begin{remark}
By combining Lemma ~\ref{xos-self} and Claim ~\ref{xos}, we immediately get that $f$ is self-bounding, and, thus, by Theorem ~\ref{bml}, it is well concentrated around its expectation.
\end{remark}
}






















% \begin{enumerate}
%     \item $\bw(\tilde{\cI}^\prime) \leq \eta_1 W$
%     \item $W_{b(\bw)}/\eta_2\leq \bw(\tilde{\cI}^\prime)$
% \end{enumerate}
% for two constants $\eta_1, \eta_2 > 1$ such that $\eta_1\eta_2 = \eta$. For (1), we can apply Claim ~\ref{talagrand} since $\bw$ is a convex $1$-Lipschitz function by Claims ~\ref{addw-lipschitz}, ~\ref{addw-convex}. Let us choose the parameter in Talagrand's Inequality $\zeta = \frac{1}{T}\left(\eta_1\left(1 - \frac{1}{c}\right) - 1\right)\E\left[\bw(\tilde{\cI}^\prime)\right] \geq c\left(\eta_1\left(1 - \frac{1}{c}\right) - 1\right) \geq c/2$, for $c \geq 2$ and $\eta_1 = 3$. Therefore,
% \begin{align}\label{upper}
%     \Pr\left[\bw(\tilde{\cI}^\prime) \leq 3 W\right] \geq \Pr\left[\bw(\tilde{\cI}^\prime) \leq \frac{3}{2} \E\left[\bw(\tilde{\cI}^\prime)\right]\right] \geq 1 - 4e^{-\frac{c^2}{16}}
% \end{align}
% For (2), we employ Claim ~\ref{talagrand} once again and choose the parameter in Talagrand's Inequality to be $\zeta = \frac{1}{T}\left(1 - \frac{1}{\eta_2}\right) \E\left[\bw(\tilde{\cI}^\prime)\right] \geq c\left(1 - \frac{1}{\eta_2}\right) \geq c/2$, for $\eta_2 = 2$. Then,
% \begin{align}\label{lower}
%     \Pr\left[\frac{W_{b(\bw)}}{2}\leq \bw(\tilde{\cI}^\prime)\right] \geq 1 - 4e^{-\frac{c^2}{16}}
% \end{align}
% By union bound on ~\ref{upper} and ~\ref{lower}, we get 
% \begin{align*}
%     \Pr\left[W_{b(\bw)} \leq 6 W\right] \geq 1 - 8e^{-\frac{c^2}{16}} \geq 1 - \frac{\beta}{\nu}
% \end{align*}
% where we have chosen $c \geq 4\sqrt{\log\left(\frac{8\nu}{\beta}\right)} $. This concludes the proof as $\eta_1\eta_2 = \eta$ and as we observe that the above is, in fact, the probability that $S$ is a good string, by definition of ``good" set.
\begin{claim}
For $\delta, \lambda \geq 1$ and $0 < \nu \leq 1$ appropriately defined constants, and $\cI^\prime, \tilde{\cI}^\prime$ as in Definitions ~\ref{optprime}, ~\ref{opttilde}. We have
\begin{align}
    \Pr\left[\bw(\tilde{\cI}^\prime) \leq \delta W \given e_t \text{ is feasible}, w_t > \tau_t\right] \geq \frac{\lambda - 1}{\lambda} \cdot \frac{\nu + \beta - 1}{\beta}
\end{align}
\end{claim}

\begin{proof}[Old proof of ~\ref{opt-lemma}]
By the way $\tilde{\cI}^\prime$ is defined, conditioning on $w_t > \tau_t$ is irrelevant for random variable $\bw(\tilde{\cI}^\prime)$, as the latter does not depend on the weight of $e_t$. Secondly, let us define the following random Boolean string $S$ encoding whether or not each element weight is above its threshold between time step $1$ and $t-1$:
\begin{align*}
    S := \left\{\bone_{w_s > \tau_s} \mid s \in [t-1]\right\}
\end{align*}
Similarly, let $\cG$ be the set of ``good" Boolean strings, i.e.
\begin{align*}
    \cG := \left\{b \in \{0,1\}^{t-1} \given \E\left[\bw(\tilde{\cI}^\prime) \mid S = b\right] \leq \eta W\right\}
\end{align*}
Hence, we can write
\begin{align*}
    \Pr&\left[\bw(\tilde{\cI}^\prime) \leq \delta W \mid e_t \text{ is feasible}, w_t > \tau_t \right] \\
    &\geq \sum_{b \in \cG}{\Pr\left[\bw(\tilde{\cI}^\prime) \leq \delta W \mid S = b, e_t \text{ is feasible}\right] \cdot \Pr[S = b \mid e_t \text{ is feasible}]}\\
    &= \sum_{b \in \cG}{\Pr\left[\bw(\tilde{\cI}^\prime) \leq \delta W \mid S = b\right] \cdot \Pr[S = b \mid e_t \text{ is feasible}]}\\
    &\geq \frac{\lambda-1}{\lambda} \cdot \sum_{b \in \cG}{\Pr[S = b \mid e_t \text{ is feasible}]} = \frac{\lambda-1}{\lambda} \cdot \Pr[S \in \cG \mid e_t \text{ is feasible}]
\end{align*}
The equality follows from the fact that $\bw(\tilde{\cI}^\prime)$ is independent of ``$e_t \text{ is feasible}$" once we condition on $S$ being a ``good" fixed Boolean string $b$. The last inequality derives from the fact that, if $S = b$, for $b \in \cG$, then by Markov's inequality and letting $W_b := \E\left[\bw(\tilde{\cI}^\prime) \mid S = b\right]$,
\begin{align*}
    \Pr\left[\bw(\tilde{\cI}^\prime) \leq \lambda\eta W \given S = b\right] &\geq \Pr\left[\bw(\tilde{\cI}^\prime) \leq \lambda W_b \given S = b\right] \geq 1 - \frac{1}{\lambda}
\end{align*}
so that $\delta=\lambda\eta$. What is left to be shown is that $\Pr[S \in \cG \mid e_t \text{ is feasible}]$ is also at least constant. Let us first observe that $\Pr\left[S \in \cG\right]$ is at least a constant. Indeed, assume the contrary, i.e. $\Pr\left[S \in \cG\right] < \nu$, then we get the following contradiction
\begin{align*}
    \E\left[\bw(\tilde{\cI}^\prime)\right] &\geq \E\left[\bw(\tilde{\cI}^\prime) \mid S \not\in \cG \right]\Pr\left[S \not\in \cG\right] \\
    &> \eta(1-\nu)\E\left[\bw(\cI^\prime)\right]
    \geq \eta(1-\nu)\left(\E\left[\bw(\tilde{\cI}^\prime)\right]-T\right) \\
    &\geq \eta(1-\nu)(1 - 1/c) \E\left[\bw(\tilde{\cI}^\prime)\right] \geq \E\left[\bw(\tilde{\cI}^\prime)\right]
\end{align*}
The third to last inequality follows from the fact that, by Claim ~\ref{lipschitzclaim}, the expected weight of $\cI^\prime, \tilde{\cI}^\prime$ can differ by at most $T$. The second to last inequality follows from the assumption that that $\E\left[\bw(\cI^\prime)\right] > cT$. Finally, for the last inequality we choose the constants such that $\eta(1-\nu)(1 - 1/c) \geq 1$. By the above, we can thus write
\begin{align*}
    \nu &\leq \Pr\left[S \in \cG\right] \\
    &= \Pr\left[S \in \cG \mid e_t \text{ is feasible}\right] \cdot \Pr\left[e_t \text{ is feasible}\right] + \Pr\left[S \in \cG \mid e_t \text{ is unfeasible}\right] \cdot \Pr\left[e_t \text{ is unfeasible}\right]\\
    &\leq \Pr\left[S \in \cG \mid e_t \text{ is feasible}\right] \cdot \Pr\left[e_t \text{ is feasible}\right] + 1 - \Pr\left[e_t \text{ is feasible}\right]
\end{align*}
Rearranging,
\begin{align*}
    \Pr\left[S \in \cG \mid e_t \text{ is feasible}\right] \geq \frac{\nu + \Pr\left[e_t \text{ is feasible}\right] - 1}{\Pr\left[e_t \text{ is feasible}\right]} \geq \frac{\nu + \beta - 1}{\beta}
\end{align*}
where the last inequality follows from the OCRS guarantee to have element $e_t$ feasible with probability at least $\beta$ by Claim ~\ref{ocrs-feasibility}. All in all, 
\begin{align*}
    \Pr\left[\bw(\tilde{\cI}^\prime) \leq \delta W \given e_t \text{ is feasible}, w_t > \tau_t\right] \geq \frac{\lambda-1}{\lambda} \cdot \frac{\nu + \beta - 1}{\beta}
\end{align*}
and the claim follows.
\end{proof}

\subsection{A Fractional Approximation}
\subsubsection{Description} The idea of the fractional approximation algorithm is based on whether there appears a ``superstar" element (an element whose weight is larger than $T$). Loosely, if at least one of such edges appears in expectation, we select the first. Otherwise, we select each edge with probability equal to the the probability it will appear in the conditionally optimal solution, i.e. $y_e$.

\RestyleAlgo{ruled}

\begin{algorithm}
\caption{Fractional Approximation}\label{fM}
\KwData{Function $w$, ground set $E$ and distributions $D_e$}
\KwResult{Subset $\cI_{\fapx} \subseteq E$ (not necessarily feasible)}
$T, D_e^\prime, \OPT^\prime, \cI^\prime, y_e$ defined as above\;
$\cI_{\fapx} \gets \emptyset$\;
\eIf{$\E\left[\bw(\cI^\prime)\right] \leq cT$}
{
    Select first element $e \in E$ such that $w_e \geq T$\;
    $\cI_{\fapx} \gets \cI_{\fapx} \cup \{e\}$\;
}{
    Set thresholds $\tau_e$ so that $\Pr\left[w_e > \tau_e\right] = y_e$\;
    Select each element $e \in E$ if $w_e > \tau_e$\;
    $\cI_{\fapx} \gets \cI_{\fapx} \cup \{e\}$\;
}
\end{algorithm}

\subsubsection{Analysis} 

Before the analysis of Algorithm ~\ref{fM}, let us show a number of small facts which will prove useful in the remainder.

\begin{claim}[Jensen's Inequality]
Let $x$ be a random variable and $g$ be any function, then
\begin{align*}
    g\left(\E\left[x\right]\right) &\leq \E\left[g(x)\right], \text{ if } g \text{ is convex.}\\
    g\left(\E\left[x\right]\right) &\geq \E\left[g(x)\right], \text{ if } g \text{ is concave.}
\end{align*}
\end{claim}

\begin{claim}
Let $a > 0$ be a constant, and $x, y > 0$ two independent random variables, then we have
\begin{align*}
    \frac{a}{a+\E\left[x\right]} &\leq \E\left[\frac{a}{a+x}\right]\\
    \frac{\E\left[x\right]}{a+\E\left[y\right]} &\leq \E\left[\frac{x}{a+y}\right]\\
\end{align*}
\end{claim}
\begin{proof}
The first inequality is a direct consequence of Jensen's Inequality (Claim ~\ref{jensen-orig}) with function $g(x) = a/(a+x)$ which is convex. The second inequality above holds because by independence of $x,y$, we have
\begin{align*}
    \E\left[\frac{x}{a+y}\right] = \E\left[x\right] \cdot \E\left[\frac{1}{a+y}\right] \geq \frac{\E\left[x\right]}{a+\E\left[y\right]}.
\end{align*}
where the last step follows again from Jensen's Inequality. 
\end{proof}

\begin{claim}
For any collection of $p_1, \dots, p_n \in (0, 1)$, let $p := \left(\prod_{i \in [n]}{p_i}\right)^{1/n}$. We have that \begin{align*}
    n\cdot\frac{1-p}{p} \leq \sum_{i \in [n]}{\frac{1-p_i}{p_i}}
\end{align*}
\end{claim}
\begin{proof}
Let us consider the base case for $p_1, p_2 \in (0,1)$: 
\begin{align*}
    \frac{2(1-\sqrt{p_1p_2})}{\sqrt{p_1p_2}} \leq \frac{1 - p_1}{p_1} + \frac{1 - p_2}{p_2}
\end{align*}

We now obtain the following,

\begin{align*}
\frac{n(1-p)}{p} &= n \cdot \frac{1 - e^{\log\left(\prod_{i \in [n]}{p_i}\right)^{1/n}}}{e^{\log\left(\prod_{i \in [n]}{p_i}\right)^{1/n}}} = n \cdot \frac{1 - e^{\frac{1}{n}\sum_{i \in [n]}{\log p_i}}}{e^{\frac{1}{n}\sum_{i \in [n]}{\log p_i}}} \\
& \leq n \cdot \frac{1 - 1/n\sum_{i\in[n]}{p_i}}{1/n\sum_{i\in[n]}{p_i}}\\
& \leq \sum_{i \in [n]}{\frac{1-p_i}{p_i}}
\end{align*}

Hereby, the first inequality is a consequence of the AM-GM inequality. 
\end{proof}

We are now ready to analyze the Algorithm ~\ref{fM} outlined above.

\begin{lemma}
For any set of distributions $\{D_e\}_{e \in E}$,
\begin{align}
    \Pr\left[\exists! \ e \in E: \ w_e > T\right] \geq \gamma \cdot \log\left(\frac{1}{\gamma}\right)
\end{align}
where the symbol ``$\exists !$" signifies the existence if a unique such element. \tec{I think we would want to quote this lemma instead of reproving. If we don't find an exact lemma that proves it, we need to say that we follow paper XXX to establish it before proving it.}
\end{lemma}

\begin{proof}
By the way we have defined $T$, we have $\Pr\left[T > \max_{e \in E}{w_e}\right] = \gamma$. This is equivalent to saying
\begin{align*}
    \Pr\left[\forall \ e \in E: \ w_e \leq T\right] = \gamma
\end{align*}
We immediately notice that the probability of the complement of above is the same as the probability of at least one $w_e$ with value at least $T$,
\begin{align*}
    \Pr\left[T < \max_{e \in E}{w_e}\right] = \Pr\left[\exists \ e \in E: \ w_e > T\right]
\end{align*}

We also know that the RHS can be written as follows by union bound of disjoint events: letting $p_e := \Pr\left[w_e < T\right]$,
\begin{align*}
    \Pr\left[\exists \ e \in E: \ w_e > T\right] &\geq \Pr\left[\exists ! \ e \in E: \ w_e > T\right] \\
    &= \sum_{e \in E}{\left((1-p_e)\cdot \prod_{e^\prime \neq e}{p_{e^\prime}}\right)} \\
    &= \prod_{e \in E}{p_e} \cdot \sum_{e \in E}{\frac{1-p_e}{p_e}}
\end{align*}

Hereby, the first equality follows from the fact that events of the form ``$\exists ! \ e \in E: \ w_e > T$" are disjoint, and the union bound holds with equality. Let us note that the threshold is larger than the maximum over all realizations if and only if all $w_e$'s realize in a value less than the threshold $T$, which happens by definition with probability $\gamma$, which means that $\prod_{e \in E}{p_e} = \gamma$. By Claim~\ref{avg-pb}, we let $p := \left(\prod_{e \in E}{p_e}\right)^{1/|E|}$ and get
\begin{align*}
     \sum_{e \in E}{\frac{1-p_e}{p_e}} &\geq |E| \cdot \frac{(1-p)}{p} \\
     &\geq |E| \cdot \frac{1-\gamma^{1/|E|}}{\gamma^{1/|E|}} \geq \log\left(\frac{1}{\gamma}\right)
\end{align*}

The second inequality follows from noticing again that $p = \gamma^{1/|E|}$, while the third by observing that the LHS of the same inequality is non-increasing in $|E|$ and the smallest value is attained for $|E| \rightarrow \infty$. All in all, we get that 
\begin{align*}
    \Pr\left[\exists ! \ e \in E: \ w_e > T\right] \geq \gamma \cdot \log\left(\frac{1}{\gamma}\right)
\end{align*}
and the statement follows.
\end{proof}

\begin{theorem}
Algorithm ~\ref{fM} produces a (potentially unfeasible) solution set $\cI_{\fapx}$ such that
\begin{align}
    \E\left[\frac{\bw(\cI_{\fapx})}{\bw(\cI^*)}\right] \geq \min\left\{\frac{\gamma \cdot \log\left(1/\gamma\right)}{c+1}, \frac{\gamma c}{c+1}\right\}
\end{align}
\end{theorem}
\begin{proof}
We divide the proof into two cases, i.e. cases where the subset of elements selected by $\OPT^\prime$ has a bounded weight in expectation as opposed to when it has a large weight. To be precise let us have the following case distinction.

\paragraph{Case 1: $\E\left[\bw(\cI^\prime)\right] \leq cT$} In this scenario, we know that the fractional competitive Algorithm ~\ref{fM} will select the first element $e \in E$ such that $w_e \geq T$. It may so happen that no such element exists in which case the fractional algorithm gets a contribution to the $\EoR$ of $0$. On the other hand, with probability $\gamma \cdot \log\left(1/\gamma\right)$, there exists exactly one edge whose weight is at least as large as $T$, by what shown in Lemma ~\ref{gamma-lemma}. Then, Algorithm ~\ref{fM} surely (with probability $1$) gets such an edge and we have
\begin{align*}
    \frac{\bw(\cI_{\fapx})}{\bw(\cI^*)} &\geq \frac{w_e}{w_e + \bw(\cI^\prime)}\\
    &\geq \frac{T}{T + \bw(\cI^\prime)}
\end{align*}
Here, the first inequality follows from Claim ~\ref{opts}, and the second by observing that since $w_e > T$, the worst possible case for the ratio is when both the $w_e$ in the numerator and the denominator are equal to $T$. Hence, with probability $\gamma \cdot \log\left(1/\gamma\right)$,
\begin{align*}
    \E\left[\frac{\bw(\cI_{\fapx})}{\bw(\cI^*)}\right] &\geq  \E\left[\frac{T}{T + \bw(\cI^\prime)}\right] \\
    &\geq \frac{T}{T + \E\left[\bw(\cI^\prime)\right]} \geq \frac{1}{c+1}
\end{align*}
The second inequality follows directly from Claim ~\ref{jensen}, whilst the last inequality derives from the assumption that $\E\left[\bw(\cI^\prime)\right] \leq cT$. To summarize, the expected competitive ratio of Case 1 reads
\begin{align*}
    \frac{\gamma \cdot \log\left(1/\gamma\right)}{c+1}
\end{align*}

\paragraph{Case 2: $\E\left[\bw(\cI^\prime)\right] > cT$} In this setting, Algorithm ~\ref{fM} selects edge $e \in E$ if $w_e > \tau_e$, which happens with probability $y_e$. If there is some edge whose weight exceeds $T$, we conservatively assume that the contribution to the expected competitive ratio will be $0$. Thus, with probability at least $\gamma$, all edges will have $w_e \leq T$. Then, since the right summand of Claim ~\ref{opts} will be $0$, we have that
\begin{align*}
    \frac{\bw(\cI_{\fapx})}{\bw(\cI^*)} &= \frac{\bw(\cI_{\fapx})}{\bw(\cI^\prime)} \\
    &\geq \sum_{e \in E}{\frac{w_e \cdot \bone[w_e > \tau_e]}{w_e \cdot \bone[w_e > \tau_e] + \bw(\cI^\prime\setminus\{e\})}}\\
    &\geq \sum_{e \in E}{\frac{w_e \cdot \bone[w_e > \tau_e]}{T + \bw(\cI^\prime)}}
\end{align*}
where, we have simply split the numerator in the sum of its terms and the denominator by isolating the weight of edge $e$. By a similar argument to the one in Case 1, we can say that the denominator is upper bounded by $T + \bw(\cI^\prime)$, reminding ourselves that random variables $\bw(\cI^\prime)$ and $w_e \cdot \bone[w_e > \tau_e]$ are completely independent. If we now take expectations around both sides of the inequality and apply Claim ~\ref{jensen}, we get
\begin{align*}
    \E\left[\frac{\bw(\cI_{\fapx})}{\bw(\cI^*)}\right] &\geq \E\left[\sum_{e \in E}{\frac{w_e \cdot \bone[w_e > \tau_e]}{T + \bw(\cI^\prime)}}\right]\\
    &\geq \frac{\E\left[\sum_{e \in E}{w_e \cdot \bone[w_e > \tau_e]}\right]}{T + \E\left[\bw(\cI^\prime)\right]} = \frac{\E\left[\bw(\cI^\prime)\right]}{T + \E\left[\bw(\cI^\prime)\right]} \\
    &\geq \frac{cT}{(c+1)T} = \frac{c}{c+1}
\end{align*}
where the last inequality follows by the assumption of Case 2. In conclusion, we get a contribution to the expected competitive ratio of
\begin{align*}
    \frac{\gamma c}{c+1}
\end{align*}
This concludes the proof. \\

{\color{red} Below might be false because OCRS are also dependent on the feasibility sets. In other words, it does not suffice to remove $e$ from $\cI^\prime$ and rerun $\OPT^\prime$ on a fresh $w_e$, because selecting $e$ might have positively or negatively affected the selection of other elements according to the feasibility constraints we impose.\\

We now apply the OCRS with approximation factor $\beta$ that turns the (possibly) unfeasible set into a feasible one. All in all, from Case 2 we get a contribution to the expected competitive ratio of
\begin{align*}
    \frac{\gamma c \beta}{c+1}
\end{align*}
To conclude the proof, we notice that the fractional algorithm achieves the best \textcolor{teal}{ATD: at least the minimum} of the two contributions to the expected competitive ratio, and thus, we can equalize them to obtain that $\gamma = e^{-c\beta}$. If we plug this value of $\gamma$ into Case 2 expression (wlog), we obtain an expected competitive ratio of
\begin{align*}
    \E\left[\frac{\bw(\cI_{\fapx})}{\bw(\cI^*)}\right] \geq \frac{e^{-c\beta}c\beta}{c+1}
\end{align*}
The RHS is maximized for $c = 1/2\left(\sqrt{(4 + \beta)/\beta} - 1\right)$, and the attained value is therefore
\begin{align*}
    \E\left[\frac{\bw(\cI_{\fapx})}{\bw(\cI^*)}\right] \geq \frac{\beta\left(\sqrt{\frac{4+\beta}{\beta}} - 1\right)e^{-\frac{\beta}{2}\left(\sqrt{\frac{4+\beta}{\beta}} - 1\right)}}{\sqrt{\frac{4+\beta}{\beta}}+1}
\end{align*}
}
\end{proof}

\begin{lemma}\label{lem:constant_reduction}
For $\beta^\prime \geq \frac{1 - p \cdot \Pr\left[e_t \text{ is feasible}\right]}{(1-p) \cdot \Pr\left[e_t \text{ is feasible}\right]}$ it holds that
\end{lemma}

\begin{proof}
It suffices to show that 
\begin{align}\label{opt-cond}
    \E \left[\bw(\cI^\prime) \mid e_t \in I, w_t > \tau_t \right] \leq \frac{1}{\beta^\prime} \cdot \E \left[\bw(\cI^\prime) \mid e_t \not\in I, w_t > \tau_t \right], \ \forall e_t \in E, t \in [T]
\end{align}
This is due to the fact that, if the above were the case, then
\begin{align*}
    \E \left[\bw(\cI^\prime)\right] &= \E \left[\bw(\cI^\prime) \mid e_t \in \cI \right] \cdot \Pr\left[e_t \in \cI \right] + \E \left[\bw(\cI^\prime) \mid e_t \not\in \cI \right] \cdot \Pr\left[e_t \not\in \cI \right] \\
    &\geq (1 + \beta^\prime) \cdot \E \left[\bw(\cI^\prime) \mid e_t \in \cI \right]
\end{align*}
and the claim would follow. Hence, let us first note that for the left-hand side in ~\ref{opt-cond}, we have that
\begin{align}\label{left_condition}
    \E \left[\bw(\cI^\prime) \mid e_t \in \cI, w_t > \tau_t \right] &= \E \left[\bw(\cI^\prime) \mid e_t \text{ is feasible}, w_t > \tau_t \right] \notag \\
    &= \frac{\E \left[\bw(\cI^\prime) \cdot \bone_{e_t \text{ is feasible}} \cdot \bone_{w_t > \tau_t} \right]}{\Pr\left[e_t \text{ is feasible}\right] \cdot \Pr\left[w_t > \tau_t \mid e_t \text{ is feasible} \right]} \;,
\end{align}
where the first equality holds since the value of $\bw(\cI^\prime)$ does not depend on the outcome of the (biased) coin flip that determines whether an element will be selected, given that it is above its threshold.

For the right-hand side in ~\ref{opt-cond}, we can decompose the conditional expectation as follows: 
\begin{align*}
    \E \left[\bw(\cI^\prime) \mid e_t \not\in \cI, w_t > \tau_t \right] &= \frac{\E \left[\bw(\cI^\prime) \cdot \bone_{e_t \not\in \cI} \cdot \bone_{w_t > \tau_t} \right]}{\Pr\left[e_t \not\in \cI \right] \cdot \Pr\left[w_t > \tau_t \mid e_t \not\in \cI \right]} \\
    &= \frac{\E \left[\bw(\cI^\prime) \cdot \bone_{e_t \text{ is feasible}} \cdot \bone_{e_t \not\in \cI} \cdot \bone_{w_t > \tau_t} \right] + \E \left[\bw(\cI^\prime) \cdot \bone_{e_t \text{ is not feasible}} \cdot \bone_{w_t > \tau_t} \right]}{\Pr\left[e_t \not\in \cI \right] \cdot \Pr\left[w_t > \tau_t \mid e_t \not\in \cI \right]} \\
    &\geq \frac{\E \left[\bw(\cI^\prime) \cdot \bone_{e_t \text{ is feasible}} \cdot \bone_{e_t \not\in \cI} \cdot \bone_{w_t > \tau_t} \right]}{\Pr\left[e_t \not\in \cI \right] \cdot \Pr\left[w_t > \tau_t \mid e_t \not\in \cI \right]} \\
    &= \frac{\E \left[\bw(\cI^\prime) \cdot \bone_{e_t \text{ is feasible}} \cdot \bone_{w_t > \tau_t} \right] \cdot (1-p)}{\Pr\left[e_t \not\in \cI \right] \cdot \Pr\left[w_t > \tau_t \mid e_t \not\in \cI \right]},
\end{align*}

where for the last equality the algorithm decides independently with probability $p$ whether to include a feasible element in the solution. Next, note that 
\[
\Pr\left[w_t > \tau_t \mid e_t \text{ is feasible} \right] = \Pr\left[w_t > \tau_t \mid e_t \not\in \cI \right]
\]
and combining with ~\ref{left_condition} we get

\[
\E \left[\bw(\cI^\prime) \mid e_t \not\in \cI, w_t > \tau_t \right] \geq \frac{\E \left[\bw(\cI^\prime) \mid e_t \in \cI, w_t > \tau_t \right] \cdot \Pr\left[e_t \text{ is feasible}\right] \cdot (1-p)}{\Pr\left[e_t \not\in \cI \right]}.
\]

Thus, to prove the lemma it suffices to select $\beta^\prime$ such that 

\[
\Pr\left[e_t \not\in \cI \right] \leq \Pr\left[e_t \text{ is feasible}\right] \cdot \beta^\prime \cdot (1-p).
\]

To relate the two probabilities, observe that 

\begin{align*}
    \Pr\left[e_t \not\in \cI \right] &= \Pr \left[e_t \text{ is feasible and } e_t \not\in \cI \right] + \Pr \left[e_t \text{ is not feasible} \right] \\
                                     &= (1-p) \Pr\left[e_t \text{ is feasible}\right] + \left(1 - \Pr\left[e_t \text{ is feasible}\right] \right) = 1 - p \cdot \Pr\left[e_t \text{ is feasible}\right] 
\end{align*}
Therefore, $\beta^\prime$ needs to satisfy

\[
 \beta^\prime \geq \frac{1 - p \cdot \Pr\left[e_t \text{ is feasible}\right]}{(1-p) \cdot \Pr\left[e_t \text{ is feasible}\right]},
\]
and the proof is complete.
\end{proof}

\begin{align*}
        &\E_{\bw, \bI}\left[\frac{\bw(\cI)}{\bw(\cI^\prime)}\right] = \E_{\bw, \bI}\left[\frac{\bw(\cI)}{\bw(\cI^\prime)}\right] = \sum_{t \in [T]}{\E_{\bw, \bI}\left[\frac{w_t \cdot \bone_{e_t \in \cI}}{\bw(\cI^\prime)} \right]} \stackrel{\text{(a)}}{\geq} \sum_{t \in [T]}{\E_{\bw, \bI}\bigg[\frac{w_t \cdot \bone_{e_t \in \cI}}{T + \bw(\underbrace{\cI^\prime\setminus\{e_t\} \cup \{\tilde{e}_t\}}_{\tilde{\cI}^\prime})}\bigg]}\\ 
        &= \sum_{t \in [T]}{\E_{\bw, \bI}\left[\frac{w_t \cdot \bone_{e_t \text{ is feasible}} \cdot \bone_{w_t > \tau_t} \cdot \bone_{\beta\text{-coin}} \cdot \bone_{p\text{-coin}}}{T + \bw(\tilde{\cI}^\prime)}\right]}\\
        &\stackrel{\text{(b)}}{=} p \cdot \sum_{t \in [T]}{\E_{\bw, \bA}\left[\frac{w_t \cdot \bone_{w_t > \tau_t} \cdot \bone_{\beta\text{-coin}}}{T + \bw(\tilde{\cI}^\prime)} \ \given \ e_t \text{ is feasible}\right]} \cdot \Pr_{\bw, \bI}\left[e_t \text{ is feasible}\right]\\
        &\stackrel{\text{(c)}}{\geq} p \cdot \sum_{t \in [T]}{\E_{\bw, \bA}\left[w_t \cdot \bone_{w_t > \tau_t} \cdot \bone_{\beta\text{-coin}} \ \given \ e_t \text{ is feasible}\right] \cdot \Pr_{\bw, \bA}\left[e_t \text{ is feasible}\right] \cdot \E_{\tilde{\bw}}\left[\frac{1}{T + \bw(\tilde{\cI}^\prime)} \ \given \ e_t \text{ is feasible}\right]}\\
        &\stackrel{\text{(d)}}{\geq} p\beta^\prime \cdot \sum_{t \in [T]}{\E_{\bw, \bA}\left[w_t \cdot \bone_{w_t > \tau_t} \cdot \bone_{\beta\text{-coin}} \ \given \ e_t \text{ is feasible}\right] \cdot \Pr_{\bw, \bA}\left[e_t \text{ is feasible}\right] \cdot \E_{\tilde{\bw}}\left[\frac{1}{T + \bw(\tilde{\cI}^\prime)}\right]}\\
        &\stackrel{\text{(e)}}{=} p\beta^\prime \cdot \E_{\bw, \bA}\left[\bw(\cA)\right] \cdot \E_{\tilde{\bw}}\left[\frac{1}{T + \bw(\tilde{\cI}^\prime)}\right]\\
        &\stackrel{\text{(f)}}{\geq} p \beta^\prime \beta\cdot \E_{\bw}\left[\bw(\tilde{\cI}^\prime)\right] \cdot \E_{\tilde{\bw}}\left[\frac{1}{T + \bw(\tilde{\cI}^\prime)}\right] \stackrel{\text{(g)}}{\geq} p \beta^\prime \beta \cdot \frac{\E_{\bw}\left[\bw(\tilde{\cI}^\prime)\right]}{T + \E_{\bw}\left[\bw(\tilde{\cI}^\prime)\right]} \\
        &\stackrel{\text{(h)}}{\geq} p \beta^\prime \beta\cdot \frac{cT}{(c+1)T} = \frac{c p}{c+1}\beta^\prime\beta 
\end{align*}
Hereby,
\begin{itemize}
    \item[] (a): We increase the denominator by $w_t$ and make $\OPT^\prime$ run on a fresh instance of $e_t$, say $\tilde{e}_t$ with weight $\tilde{w}_t$ samples from the same distribution of $w_t$, while leaving all the remaining weights unaltered. The denominator is upper bounded by $T + \bw(\cI^\prime)$.
    \item[] (b): We notice that the $p$-coin indicator is independent of all other random variables in the expectation expression.
    \item[] (c): From (a), random variables $\bw(\cI^\prime)$ and $w_t$ will be completely independent, since $w_t$ has been chosen by the OCRS algorithm and we have uncoupled the weight of $\cI^\prime$ from this specific realization of element $e_t$'s weight. From (b), we also notice that the optimum is independent of all indicators apart from the feasibility one, on which we condition.
    \item[] (d): This follows from Lemma ~\ref{lem:constant_reduction}.
    \item[] (e): The sum evaluates to the weight the $\beta$-OCRS algorithm achieves.
    \item[] (f): This follows from the definition of $\beta$-OCRS.
    \item[] (g): This derives by applying Jensen's inequality in the form of Claim ~\ref{jensen}.
    \item[] (h): This is the assumption of Case 2.
\end{itemize}

==> sections/old2_sc.tex <==
\section{Single-Choice $\EoR$ Prophet Inequality}

We start with the case where the distribution vector $\bF$ is known to the stopping rule $\textbf{r}$ and its components are not identical. This is essential when we assume that we can compute probabilities as well as expectations, in that it would be not possible to calculate them without full-knowledge of the distributions $F_i$.

\subsection{$\RoE$ and $\EoR$ separation: $1/e$ is tight for EoR}\label{noniid_known}

The aim of this subsection is to provide an stopping rule achieving a lower bound on the $\EoR$ of $1/e$ and show, by constructing an explicit example, that the subsequent upper bound matches exactly the lower bound.

\medskip

We hereby present a simple stopping rule that achieves an $\EoR$ of at least $1/e$, assuming without loss of generality that  all the distributions we are dealing with are continuous distributions. We will make use of the following fact.
\begin{claim}[Derived from AM-GM Inequality]\label{mult_mean}
For any collection of $p_1, \dots, p_n \in (0, 1)$, let $p := \left(\prod_{i \in [n]}{p_i}\right)^{1/n}$. We have that \begin{align*}
    n\cdot\frac{1-p}{p} \leq \sum_{i \in [n]}{\frac{1-p_i}{p_i}}
\end{align*}
\end{claim}
\begin{proof}
To start giving an intuition about the claim, consider the base case inequality for $p_1, p_2 \in (0,1)$: 
\begin{align*}
    \frac{2(1-\sqrt{p_1p_2})}{\sqrt{p_1p_2}} \leq \frac{1 - p_1}{p_1} + \frac{1 - p_2}{p_2}
\end{align*}

We now obtain the following,

\begin{align*}
\frac{n(1-p)}{p} &= n \cdot \frac{1 - e^{\log\left(\prod_{i \in [n]}{p_i}\right)^{1/n}}}{e^{\log\left(\prod_{i \in [n]}{p_i}\right)^{1/n}}} = n \cdot \frac{1 - e^{\frac{1}{n}\sum_{i \in [n]}{\log p_i}}}{e^{\frac{1}{n}\sum_{i \in [n]}{\log p_i}}} \\
& \leq n \cdot \frac{1 - 1/n\sum_{i\in[n]}{p_i}}{1/n\sum_{i\in[n]}{p_i}}\\
& \leq \sum_{i \in [n]}{\frac{1-p_i}{p_i}}
\end{align*}

Hereby, the first inequality is a consequence of the AM-GM inequality. 
\end{proof}

\begin{theorem} [Lower bound]
For any set of distributions $F_1, \dots, F_n$, there exists a stopping rule $\textbf{r}$ such that
\begin{align}
    \E\left[\frac{X_\tau}{\max_{i \in [n]}{X_i}}\right] \geq \frac{1}{e}
\end{align}
Hereby, $X_{\tau}$ is the value stopping rule $\textbf{r}$ picks.
\end{theorem}

\begin{proof}
We will use the fixed threshold stopping rule choosing $T$ such that 
\begin{align*}
    \Pr\left[T > \max_{i \in [n]}{X_i}\right] = 1/e
\end{align*}
We will prove that it achieves $\EoR \geq 1/e$. To this end, let $p_i := \Pr\left[X_i < T\right]$. We immediately notice that the probability of the complement of above is the same as the probability of at least one $X_i$ such that its value is at least $T$.\footnote{Note that we are using continuity to write event ``$T \leq \max_{i \in [n]}{X_i}$" and ``$T < \max_{i \in [n]}{X_i}$" interchangeably.} This means
\begin{align*}
    \Pr\left[T < \max_{i \in [n]}{X_i}\right] = \Pr\left[\exists \ i \in [n]: \ X_i > T\right]
\end{align*}

We also know that the RHS can be written as follows by union bound of disjoint events (the first equality, where by $\exists \ !i$ we denote that there exists a unique such $i$):\footnote{We remark that events of the form ``$\exists \ !i \in [n]: \ X_i > T$" are not pairwise independent. That is why we can do the trick below.}
\begin{align*}
    \Pr\left[\exists \ i \in [n]: \ X_i > T\right] &\geq \Pr\left[\exists \ !i \in [n]: \ X_i > T\right] \\
    &= \sum_{i \in [n]}{\left((1-p_i)\cdot \prod_{j \neq i}{p_j}\right)} \\
    &= \prod_{i \in [n]}{p_i} \cdot \sum_{i \in [n]}{\frac{1-p_i}{p_i}}
\end{align*}

Let us note that the threshold is larger than the maximum over all realizations if and only if all $X_i$'s realize in a value less than the threshold $T$, which happens by definition with probability $1/e$. This means that $\prod_{i \in [n]}{p_i} = 1/e$: to prove the theorem, it thus suffices to show that following sum is larger than $1$.
\begin{align*}
    \sum_{i \in [n]}{\frac{1-p_i}{p_i}} \geq 1
\end{align*}

In order to prove that this holds, we make use of a standard trick that shows $\sum_{i}{\frac{1-p_i}{p_i}} \geq n(1-p)/p$, where $p$ is the value obtained from the multiplicative average of $\sum_{i}{\frac{1-p_i}{p_i}}$. To be precise, as per Claim~\ref{mult_mean}, letting $p := \left(\prod_{i \in [n]}{p_i}\right)^{1/n}$, we get that
\begin{align*}
    \frac{n(1-p)}{p} \leq \sum_{i \in [n]}{\frac{1-p_i}{p_i}}
\end{align*}

Therefore if we showed that $n(1-p)/p \geq 1$, we would be done. To this end, let us recall that we still have $\prod_{i}{p_i} = 1/e$, and since $p^n = \prod_{i \in [n]}{p_i}$, then $p^n = 1/e$. Taking logarithms on both sides, we obtain $n = -1/\log p$, and substituting it into the above, we would need to show
\begin{align*}
    \frac{p-1}{p\log p} \geq 1 \ \text{ or, equivalently, } \ p-1 \leq p\log p
\end{align*}

The equivalence is given by the fact that $\log p < 0$ as $p < 1$. Thus, since the above holds for any $p \in (0,1)$, the statement follows.
\end{proof}

\begin{theorem} [Upper bound]
For a single choice online stopping problem, no stopping rule achieves $\EoR$ larger than $1/e$.
\end{theorem}
\begin{proof}
Let us consider the following collection of distributions $\bF = \{F_i\}_{i \in \{0\} \cup [n-1]}$,
\begin{align}
    F_0: \ X_0 = 1, \text{ w.p. } 1, \ F_i: \ X_i = \begin{cases}
        0, \text{ w.p. } 1 - p_i\\
        M^i, \text{ w.p. } p_i
    \end{cases}
\end{align}

Hereby, both $M = M(n)$ and $p_i = p_i(n)$  are functions of the sequence length $n$.

\begin{observation}[Case distinction]\label{obs_last}
We are interested in characterizing the distribution of $X_\tau/\max_{i \in [n]}{X_i}$, to then compute \EoR. We have three possible cases,
\begin{enumerate}
    \item $X_\tau/\max_{i \in [n]}{X_i} = 0$
    \item $X_\tau/\max_{i \in [n]}{X_i} = 1$
    \item $X_\tau/\max_{i \in [n]}{X_i} = M^{j - k}$ for some $1 \leq j < k \leq n$
\end{enumerate}
\end{observation}

We hence know that the possible values for the ratio $X_\tau/\max_{i \in [n]}{X_i}$ potentially belong to $\mathcal{V} = \{0, M^{1-n}, \dots, M^{-1}, 1\}$. Therefore,
\begin{align*}
    \EoR &= \E\left[\frac{X_\tau}{\max_{i \in [n]}{X_i}}\right] = \sum_{v \in \mathcal{V}}{v \cdot \Pr\left[\frac{X_\tau}{\max_{i \in [n]}{X_i}} = v\right]} \\
    &= 0 \cdot \Pr\left[\frac{X_\tau}{\max_{i \in [n]}{X_i}} = 0\right] + 1 \cdot \Pr\left[\frac{X_\tau}{\max_{i \in [n]}{X_i}} = 1\right] + \sum_{v \in \mathcal{V}\setminus\{0,1\}}{v \cdot \Pr\left[\frac{X_\tau}{\max_{i \in [n]}{X_i}} = v\right]}\\
    &= \EoR^{(1)} + \EoR^{(2)} + \EoR^{(3)} \\
    &\leq \EoR^{(2)} + \frac{1}{M}
\end{align*}

The idea is to take $M$ very large, so that $\EoR^{(3)} \leq 1/M$ and, thus, roughly zero (while obviously $\EoR^{(1)} = 0$). Hence, the $\EoR$ is (essentially) $\EoR^{(2)}$. We will now explain what the two contrasting sides of the model are trying to achieve: on one hand we have $\textbf{r}$ that wants to maximize the probability of being equal to $\max_{i \in [n]}{X_i}$ (even when $\textbf{r}$ and $\max_{i \in [n]}{X_i}$ are a multiplicative $M$ away, we conservatively assume their ratio is $0$). Let us, therefore, denote by $R_i$ the probability that $X_\tau/\max_{i \in [n]}{X_i} = 1$, had $\textbf{r}$ chosen threshold $T = M^i$. First of all, let us observe that 
\begin{align*}
    &R_{n-1} = p_{n-1}\\
    &R_{n-2} = p_{n-2}(1 - p_{n-1}) + (1 - p_{n-2})p_{n-1}\\
    &\vdots\\
    &R_i = \sum_{j \geq i}{\left(p_j \cdot \prod_{\substack{k > i\\k\neq j}}{(1 - p_k)}\right)} = \sum_{j \geq i}{\left(\frac{p_j}{1 - p_j} \cdot \prod_{k \geq i}{(1 - p_k)}\right)} = \prod_{k \geq i}{(1 - p_k)} \cdot \sum_{j \geq i}{\frac{p_j}{1 - p_j}}\\
    &\vdots\\
    &R_1 = \prod_{k \geq 1}{(1 - p_k)} \cdot \sum_{j \in [n-1]}{\frac{p_j}{1 - p_j}}\\
    &R_0 = \prod_{k \geq 1}{(1 - p_k)}
\end{align*}

This is indeed easy to see: if $\textbf{r}$ chose threshold $T = M^n$, then the only possibility it has to equal $\max_{i \in [n]}{X_i}$ would be realizing at the last instance. Choosing $T = M^{n-1}$, $\textbf{r}$ can equal $\max_{i \in [n]}{X_i}$ if either they both realize in $X_{n-1}$ or both in $X_{n}$; this means that, in one case, the last instance should realize in $0$ and, in the other case, the second-to-last instance needs realize in $0$, as otherwise $\textbf{r}$ would accept it. Unrolling the induction, we see that if $\textbf{r}$ chose $M^i$, only one of the $X$'s with index at least $i$ can be nonzero, or else all the $X$'s need to be zero. Formally, we have that
\begin{align}
    R_i := \Pr\left[\frac{X_\tau}{\max_{i \in [n]}{X_i}} = 1 \ \bigg| \ T = M^i\right] = \prod_{k \geq i}{(1 - p_k)} \cdot \sum_{j \geq i}{\frac{p_j}{1 - p_j}}
\end{align}

In order for us to be able to match the above lower bound of $1/e$, let $p_i = p = 1/n$ for all $i \in \{0\} \cup [n-1]$. We can thus rewrite the general probability of being as good as $\max_{i \in [n]}{X_i}$:
\begin{align*}
    R_0 = \left(1 - \frac{1}{n}\right)^{n-1} \ \text{ and } R_i = \frac{n-i}{n} \cdot \left(1 - \frac{1}{n}\right)^{n-i-1}
\end{align*}

$\textbf{r}$'s objective is to maximize the $R_i$ expression with respect to $i$, including index $0$. It is easy to see that $R_i$ is a decreasing function of $i$ that has a minimum at $i = n-1$, i.e. $R_{n-1} = 1/n - 1/n^2$, and a maximum at $i = 0$, i.e. $R_0 = (1 - 1/n)^{n-1}$ for any $n$ (also note that for $i=n$, which is not allowed, $R_n = 0$). Asymptotically,
    \begin{align*}
        \lim_{n \to \infty}{\left(1 - \frac{1}{n}\right)^{n-1}} = \frac{1}{e}
    \end{align*}
    
We observe that the choice $p = 1/n$ matches the provided lower bound of $1/e$. We, therefore, show there exists an asymptotic separation between the constants in $\RoE$ which is $1/2$ (tightly) and the $\EoR$ one which is $1/e$.
\end{proof}

\begin{remark}
We remark that we have not employed the reduction of Theorem \ref{reduction}, but used a simple thresholding argument to prove the lower bound. If we had used it however, we could obtain the same lower bound as shown by Theorem 1 in \cite{esfandiari}, which proves a $1/e$ lower bound for the best-choice prophet inequality problem. Another hard instance is constructed in Theorem 2 of the same paper to show tightness of $1/e$.
\end{remark}

==> sections/prelim.tex <==
\section{Preliminaries}

\subsection{Feasibility constraints}
Under the lens of this new measure, we would like to explore various feasibility structures. Before delving into their description, let us describe in general what our objective will be. Let $U$ be a ground set of elements, $\cF \subseteq 2^U$ a set of constraints (also called independent family), and an objective function $f: 2^U \rightarrow \mathbb{R}$, we aim to maximize $f$ upon selecting a feasible set $S \in \cF$. In this case, $f := \EoR$ and elements $u \in U$ are (adversarially) stochastic and presented online. 

Specifically, we will focus on (a subset of) downward closed feasibility structures, that is a family of constraints such that if, for $E \supseteq E^\prime$, $E \in \cF$, then $E^\prime \in \cF$. In the following, we give a few examples of downward closed feasibility structures we would like to explore under the $\EoR$ lens.

\subsubsection{Single-choice} In this setting, $X_1 \sim D_1, \dots, X_n \sim D_n$ and our goal is to maximize the following expression, with the constraint of selecting a single value:
\begin{align*}
    \EoR := \E\left[\frac{X_\tau}{\max_{i \in [n]}{X_i}}\right]
\end{align*}
\noindent Above, we have dropped the subscripts (for ease of notation), and we express $\ALG(\bX) := X_\tau$, the value where we have decided to stop. Similarly, it is easy to see that $\OPT(\bX) = \max_{i \in [n]}{X_i}$.

\subsubsection{$k$-choice} In this setting, $X_1 \sim D_1, \dots, X_n \sim D_n$ and our goal is to maximize the following expression, with the constraint of selecting at most $k$ values:
\begin{align*}
    \EoR := \E\left[\frac{\sum_{i \in \cI}{X_i}}{\sum_{i \in \cI^*}{X_i}}\right]
\end{align*}
\noindent Above, we express $\ALG(\bX) := \sum_{i \in \cI}{X_i}$, the values we have decided to pick, which belong to some $\cI \subseteq_k [n]$. Similarly, it is easy to see that $\OPT(\bX) = \sum_{i \in \cI^*}{X_i}$, where $\cI^* \subseteq_k [n]$ of maximal total weight. This can also be seen as a $k$-uniform matroid.

\subsubsection{Maximum matching} In this setting, we have the following two possibilities:
\begin{enumerate}
    \item In the vertex arrival (V.A.) model, vertices arrive in an online fashion independently along with their incident edges, so that $\bw_v \sim D_v$ is the random vector of edge weights adjacent to $v$.
    \item In the edge arrival (E.A.) model, edges arrive in an online fashion independently, so that $w_e \sim D_e$ is the random variable denoting an edge weight.
\end{enumerate}

In both cases, our goal is to maximize the following expression, with the constraint of selecting a matching in the graph (all vertices are covered and no two edges share the same vertex):
\begin{align*}
    \EoR := \E\left[\frac{\bw(\cI)}{\bw(\cI^*)}\right]
\end{align*}
\noindent Above, we express $\ALG(\bw) := \bw(\cI)$, the weight of the matching $\cI$ we have chosen. Similarly, it is easy to see that $\OPT(\bw) = \bw(\cI^*)$, the weight of the maximum matching $\cI^*$.

\subsubsection{Matroid}
A matroid $\cM = (U, \cF)$ is a downward closed set composed of a ground set of elements $U$ (with $|U| = n$) and an independence family $\cF$ such that for any pair of independent sets $E, E^\prime \in \cF$ with $|E^\prime| \leq |E|$, there exists an element $u \in E$ for which $E^\prime \cup \{u\} \in \cF$. The latter is known as the exchange axiom.

In this setting, $u_1 \sim D_1, \dots, u_n \sim D_n$ and our goal is to maximize the following expression, with the constraint of selecting an independent set in the given matroid:
\begin{align*}
    \EoR := \E\left[\frac{\bw(E)}{\bw(E^*)}\right]
\end{align*}
\noindent Above, we express $\ALG(\bu) := \bw(E)$, the weight of the independent set $E \in \cF$ we have decided to pick. Similarly, it is easy to see that $\OPT(\bu) = \bw(E^*)$, the weight of the optimal independent set $E^* \in \cF$.

==> sections/second_reduction_old.tex <==
\subsection{Second Reduction: from \EoR { }to \RoE}
In this section, we show a reduction from  $\EoR$ to $\RoE$. 
\begin{theorem}\label{alg-analysis-rev}
For every downward-closed family of feasibility sets $\cF$, it holds that
\begin{align}
\RoE(\cF) \geq \frac{\EoR(\cF)}{18}.
\end{align}
\end{theorem}

% \begin{theorem}\label{alg-analysis-rev}
% Algorithm ~\ref{general-rev} produces a solution set $\ALG(\bw)$ such that
% \begin{align}
%     \emph{\E}\left[a(\bw)\right] \geq \frac{\alpha}{12}\emph{\E}\left[f(\bw)\right].
% \end{align}
% \end{theorem}

\RestyleAlgo{ruled}
\begin{algorithm}
\caption{$\EoR\text{-to-}\RoE$}\label{general-rev}
\KwData{Ground set $E$, distributions $D_e$, feasibility family $\cF$, a subroutine $\ALGEOR$ }
\textbf{Assumption:} $\ALGEOR(\bw)$ satisfies that $\E_{\bw \sim D}\left[a_{\ALGEOR}(\bw)/f(\bw) \mid \cE_0 \right] \geq \alpha$

\textbf{Parameters:} $\gamma \in (0,1)$, $\ell<1$, $r > 0$

\KwResult{Subset $\ALG(\bw) \subseteq E$ such that
$\ALG(\bw) \in \cF$}
Calculate $\tau$ according to Equation~\eqref{eq:t}\;
Calculate $W:=\E\left[f(\overline{\bw})\right]$\;

\eIf{$W \leq \max\{\ell \cdot \emph{\E}\left[f(\bw)\right],  r \cdot \tau\}$}
{
    Return the first element $e^* \in E$ such that $w_{e^*} \geq \tau$\;
    %$\ALG(\bw) \gets \{e\}$\;
    If no such element exists, return $\emptyset$\;
}{
    As long as $w_e \leq \tau$ run
    $\ALGEOR(\bw)$\;
    If $w_e > \tau$, reject all remaining elements\;
}
\end{algorithm}

% \begin{algorithm}
% \caption{$\EoR\text{-to-}\RoE$}\label{general-rev}
% \KwData{Ground set $E$, distributions $D_e$, feasibility family $\cF$}
% \KwResult{Subset $\ALG(\bw) \subseteq E$ such that $\ALG(\bw) \in \cF$}
% $\ALG(\bw) \gets \emptyset$\;
% \eIf{$W \leq \ell \emph{\E}\left[f(\bw)\right]$ \emph{\textbf{or}} $W \leq r T$}
% {
%     Select first element $e \in E$ such that $w_e \geq \tau$\;
%     $\ALG(\bw) \gets \ALG(\bw) \cup \{e\}$\;
% }{
%     $\ALG(\bw) \gets \ALGEOR(\bw)$\;
% }
% \end{algorithm}

Similarly to the proof of \Cref{alg-analysis}, we will assume the existence of an algorithm $\ALGEOR(\bw)$ that satisfies  
\begin{equation}
    \E_{\bw \sim D}\left[\frac{a_{\ALGEOR}(\bw)}{f(\bw)} \given \cE_0 \right] = \E_{\overline{\bw} \sim \overline{D}}\left[\frac{a_{\ALGEOR}(\bw)}{f(\bw)}\right] \geq \alpha. \label{eq:assumption-eor}
\end{equation} 
Our analysis distinguishes between two cases; in the first case (see \Cref{lem:supeor}), one of the conditions of $W:= \E\left[f(\overline{\bw})\right] \leq \ell \cdot \E\left[f(\bw)\right]$ or $W \leq r \cdot \tau$ holds. The second case (see \Cref{lem:combeor}) analyzes the scenario where neither of the conditions hold. In the remainder, for ease of notation, we denote the expected value  of \Cref{general-rev} on $\bw$ by $ a(\bw)$.

\begin{lemma}[``Catch the superstar'']\label{lem:supeor}
For all constants $\theta, \ell \in (0,1), k \geq 1$ and $r \geq \frac{2}{\theta^2} \log \frac{k}{\alpha}$, if $W \leq \max\{ \ell \cdot \emph{\E}\left[f(\bw)\right],W \leq r \cdot \tau\}$, then \Cref{general-rev} satisfies 
\begin{align}
    \emph{\E}\left[a(\bw)\right] \geq \min\left\{\gamma(1-\ell), \frac{(1-\gamma)\ell}{r}\right\} \cdot \emph{\E}\left[f(\bw)\right].
\end{align}
\end{lemma}

\begin{proof}
In this case, \Cref{general-rev} selects the first element whose weight exceeds threshold $\tau$. As per the statement, we have the following two subcases:
\begin{enumerate}
    \item If $W \leq \ell \cdot \E\left[f(\bw)\right]$, the algorithm accepts the first element that exceeds the threshold $\tau$. Thus, the expected weight of the algorithm's output is
    \begin{align*}
        \E\left[a(\bw)\right] &= \sum_{e \in E}{\Pr[\forall e^\prime < e, \enspace  w_{e^\prime} \leq \tau ] \cdot \E\left[w_e \cdot  \bone_{w_e > \tau}\right]}\\
        &\geq \gamma \cdot \E\left[\sum_{e \in E}{w_e \cdot \bone_{w_e > \tau}}\right] \\
        &\geq \gamma \cdot \left(\E\left[f(\bw)\right] - \E\left[f(\overline{\bw})\right]\right)\\
        &\geq \gamma \cdot (1-\ell) \cdot \E\left[f(\bw)\right],
    \end{align*}
    where the first inequality derives from \Cref{gamma-lemma}, and the fact that the probability that no element exceeds $\tau$ up to the arrival of element $e$ is at least the probability that no element exceeds $\tau$ until the end. %with probability at least $\gamma$, all elements appearing before $e^\prime$ will have weight bounded above by threshold $\tau$. 
    The second inequality follows by taking the expectation over the expression in \Cref{opts}, and finally the last inequality follows from our assumption.
    \item If $W \leq r \cdot \tau$  and $W > \ell \cdot \E\left[f(\bw)\right]$, %Algorithm ~\ref{general-rev} selects the first element whose weight exceeds $\tau$, 
    then
    \begin{align*}
        \E\left[a(\bw)\right] \geq (1-\gamma) \tau \geq \frac{1-\gamma}{r} \cdot W \geq \frac{(1-\gamma)\ell}{r} \cdot \E\left[f(\bw)\right].
    \end{align*}
\end{enumerate}
This concludes the proof of the lemma.
\end{proof}

\begin{lemma}[``Run the combinatorial algorithm'']\label{lem:combeor}
For all constants $\theta, \ell \in (0,1), k \geq 1$ and $r \geq \frac{2}{\theta^2} \log \frac{k}{\alpha}$, if $W > \max\{\ell \cdot \emph{\E}\left[f(\bw)\right], r \cdot \tau\}$, then \Cref{general-rev} satisfies
\begin{align}
    \emph{\E}\left[a(\bw)\right] \geq \gamma \left(1 - \frac{1}{k}\right) \left(1-\frac{\alpha}{k}\right)\cdot \alpha(1-\theta)\ell \cdot \emph{\E}\left[f(\bw)\right].
\end{align}
\end{lemma}
\begin{proof}
In this case, since $W > \max\{\ell \cdot \E\left[f(\bw)\right],W > r \cdot \tau\} $, then  
\Cref{general-rev} runs the $\ALGEOR$ subroutine. By \Cref{prop:bounding}, we know that $f(\bw)/\tau$ is self-bounding in the domain of $[0,\tau]$, and, thus, by \Cref{blm},
\begin{align} \label{eq:low-prob}
    \Pr\left[f(\bw) \leq (1-\theta)W \mid \cE_0\right] &\leq e^{-\frac{\theta^2 W}{2T}} < e^{-\frac{\theta^2 r}{2}} \leq \frac{\alpha}{k}.
\end{align}
%where we set $r \geq \frac{2}{\theta^2} \log \frac{k}{\alpha}$. 
We also know that
\begin{align}
    \E\left[a(\bw) \mid \cE_0\right] &\geq \E\left[a(\bw) \given f(\bw) > (1-\theta)W, \cE_0\right] \cdot \Pr\left[f(\bw) > (1-\theta)W \mid \cE_0\right] \nonumber \\
    &> \left(1-\frac{\alpha}{k}\right) \cdot \E\left[a(\bw) \given f(\bw) > (1-\theta)W, \cE_0\right], \label{eq:aw} 
\end{align}
where the first inequality is by the law of total expectation, and the second inequality is by Inequality~\eqref{eq:low-prob}.
Hence,
\begin{align}
    \alpha &\leq \E\left[\frac{a(\bw)}{f(\bw)} \given \cE_0\right] = \underbrace{\E\left[\frac{a(\bw)}{f(\bw)} \given f(\bw) \leq (1-\theta)W, \cE_0\right]}_{\leq 1} \cdot \Pr\left[f(\bw) \leq (1-\theta)W \mid \cE_0\right] \nonumber\\
    &\qquad\qquad\qquad\quad + \E\left[\frac{a(\bw)}{f(\bw)} \given f(\bw) > (1-\theta)W, \cE_0\right] \cdot \underbrace{\Pr\left[f(\bw) > (1-\theta)W \mid \cE_0\right]}_{\leq 1} \nonumber \\
    &<  \frac{\alpha}{k} + \frac{\E\left[a(\bw) \mid \cE_0\right]}{(1-\theta)W} / \left(1 - \frac{\alpha}{k}\right)\nonumber \\ &\leq \frac{\alpha}{k} + \frac{\E\left[a(\bw) \mid \cE_0\right]}{(1-\theta)\ell \cdot \E\left[f(\bw)\right]}/ \left(1 - \frac{\alpha}{k}\right), \label{eq:alpha-aw}
\end{align}
where the first inequality follows by Inequality~\eqref{eq:assumption-eor}, the second inequality follows by Inequality~\eqref{eq:aw} and by replacing both $\Pr\left[f(\bw) > (1-\theta)W \mid \cE_0\right]$ and $\E\left[\frac{a(\bw)}{f(\bw)} \given f(\bw) \leq (1-\theta)W, \cE_0\right]$ by $1$, and the last inequality holds by our assumption that $W>\ell \cdot \E[f(\bw)]$.

Hence, given that $\E\left[a(\bw)\right] \geq \gamma \E\left[a(\bw) \mid \cE_0\right]$, and by rearranging  Inequality~\eqref{eq:alpha-aw}, we obtain
\begin{align*}
    \E\left[a(\bw)\right] \geq \gamma \left(1 - \frac{1}{k}\right) \left(1-\frac{\alpha}{k}\right) \cdot \alpha(1-\theta)\ell \cdot \E\left[f(\bw)\right].
\end{align*}
This concludes the proof of the lemma.
\end{proof}

\begin{proof}[Proof of \Cref{alg-analysis-rev}]
If $\alpha=\EoR(\cF)$, then there exists an algorithm $\ALGEOR$ that satisfies Equation~\ref{eq:assumption-eor}.
\Cref{general-rev} guarantees the minimum between the competitive ratios of \Cref{lem:supeor} and \Cref{lem:combeor}. Thus, we need to find parameters $\gamma,\theta,k,\ell,r$ that maximize the following  constrained optimization problem:
\begin{align*}
    \mbox{ \text{maximize} } \quad \quad& \min\left\{\gamma(1-\ell) , \frac{(1-\gamma)\ell}{r},\gamma \left(1 - \frac{1}{k}\right)\left(1-\frac{\alpha}{k}\right) \cdot \alpha(1-\theta)\ell\right\}  \\
    \text{subject to} \quad \quad & \enspace  \gamma, \theta, \ell \in (0,1), k \geq 1,  r \geq \frac{2}{\theta^2} \log \frac{k}{\alpha}.
\end{align*}
The only parameter we do not control is $\alpha$, as it depends on the feasibility structure $\cF$. Let us choose constants $\gamma = 1/2, \theta=1/2, \ell = 8/9, k=2$, and $r = 8 \log \frac{2}{\alpha} $. With this choice of parameters, for all $\alpha \in (0, 1]$, \Cref{lem:supeor} and \Cref{lem:combeor} yield $\min\left\{\frac{1}{18}, \frac{1}{18\log(2/\alpha)}, \frac{\alpha}{9} \left(1 - \frac{\alpha}{2}\right)\right\} \geq \frac{\alpha}{18}$, which concludes the proof.
\end{proof}
